Model Predictive Control for Finite Input Systems using the D-Wave Quantum Annealer

The D-Wave quantum annealer has emerged as a novel computational architecture that is attracting significant interest, but there have been only a few practical algorithms exploiting the power of quantum annealers. Here we present a model predictive control (MPC) algorithm using a quantum annealer for a system allowing a finite number of input values. Such an MPC problem is classified as a non-deterministic polynomial-time-hard combinatorial problem, and thus real-time sequential optimization is difficult to obtain with conventional computational systems. We circumvent this difficulty by converting the original MPC problem into a quadratic unconstrained binary optimization problem, which is then solved by the D-Wave quantum annealer. Two practical applications, namely stabilization of a spring-mass-damper system and dynamic audio quantization, are demonstrated. For both, the D-Wave method exhibits better performance than the classical simulated annealing method. Our results suggest new applications of quantum annealers in the direction of dynamic control problems.

==> __latexindent_temp.tex <==

@incollection{Cornejo2015Distributed,
  title = {Distributed {{Range}}-{{Based Relative Localization}} of {{Robot Swarms}}},
  booktitle = {Algorithmic {{Foundations}} of {{Robotics XI}}},
  publisher = {{Springer}},
  author = {Cornejo, Alejandro and Nagpal, Radhika},
  year = {2015},
  pages = {91-107},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed Range-Based Relative Localization of Robot Swarms.pdf}
}

@phdthesis{Barooah2007Estimation,
  address = {{Santa Barbara, CA, USA}},
  title = {Estimation and {{Control}} with {{Relative Measurements}}: {{Algorithms}} and {{Scaling Laws}}},
  school = {University of California at Santa Barbara},
  author = {Barooah, Prabir},
  year = {2007},
  file = {/Users/e1727/Dropbox/papers/storage/Estimation and Control with Relative Measurements.pdf},
  isbn = {978-0-549-27004-1},
  advisor = {Hespanha, Joao P.},
  note = {AAI3283774}
}

@article{Zhang2011MotionEstimationBased,
  title = {Motion-{{Estimation}}-{{Based Visual Servoing}} of {{Nonholonomic Mobile Robots}}},
  volume = {27},
  issn = {1552-3098},
  number = {6},
  journal = {IEEE Transactions on Robotics},
  doi = {10.1109/TRO.2011.2162765},
  author = {Zhang, X. and Fang, Y. and Liu, X.},
  month = dec,
  year = {2011},
  keywords = {estimation theory,closed loop systems,closed-loop system,Field of view (FOV),field-of-view,FOV,image sensors,matrix algebra,matrix decomposition,matrix estimation,mobile robots,Mobile robots,monocular camera systems,motion control,Motion control,motion estimation,motion estimation based visual servoing,nonholonomic mobile robots,onboard camera,parking problem,planar motion,planar motion estimation,robot vision,time-varying feedback controller,Transmission line matrix methods,visual servoing,Visual servoing,wheeled robots},
  pages = {1167-1175},
  file = {/Users/e1727/Dropbox/papers/storage/Motion-Estimation-Based Visual Servoing of Nonholonomic Mobile Robots.pdf}
}

@inproceedings{Shang2004Improved,
  title = {Improved {{MDS}}-Based Localization},
  volume = {4},
  booktitle = {{{IEEE INFOCOM}} 2004},
  doi = {10.1109/INFCOM.2004.1354683},
  author = {Shang, Yi and Ruml, W.},
  month = mar,
  year = {2004},
  keywords = {Acoustic sensors,Actuators,centralized algorithm,Communication networks,communications network,Computer science,connectivity information,Euclidean distance,geographic position,global map,Global Positioning System,irregularly-shaped network,Large-scale systems,localization method,multidimensional scaling,Multidimensional systems,Network topology,radio networks,Temperature sensors},
  pages = {2640-2651 vol.4},
  file = {/Users/e1727/Dropbox/papers/storage/Improved MDS-based localization.pdf},
  issn = {0743-166X}
}

@inproceedings{Rubenstein2012Kilobot,
  title = {Kilobot: {{A Low Cost Scalable Robot System}} for {{Collective Behaviors}}},
  booktitle = {2012 {{IEEE International Conference}} on {{Robotics}} and {{Automation}}},
  doi = {10.1109/ICRA.2012.6224638},
  author = {Rubenstein, M. and Ahler, C. and Nagpal, R.},
  month = may,
  year = {2012},
  keywords = {Robot sensing systems,Batteries,collective behaviors,Collision avoidance,decentralised control,decentralized cooperating robots,Kilobot collective,low cost scalable robot system,multi-robot systems,research and development,robot design,Robot kinematics,robotics research,Switches,testing collective algorithms},
  pages = {3293-3298},
  file = {/Users/e1727/Dropbox/papers/storage/Kilobot.pdf},
  issn = {1050-4729}
}

@article{Shang2004Localization,
  title = {Localization from {{Connectivity}} in {{Sensor Networks}}},
  volume = {15},
  issn = {1045-9219},
  number = {11},
  journal = {IEEE Transactions on Parallel and Distributed Systems},
  doi = {10.1109/TPDS.2004.67},
  author = {Shang, Y. and Rumi, W. and Zhang, Y. and Fromherz, M.},
  month = nov,
  year = {2004},
  keywords = {network localization,optimisation,wireless sensor networks,Acoustic sensors,Actuators,connectivity information,Global Positioning System,multidimensional scaling,Multidimensional systems,Temperature sensors,ad hoc networks,Ad hoc networks,communication complexity,Computational modeling,data analysis,Data analysis,Intelligent networks,irregular networks,least squares approximations,least-squares optimization,mobile communication,mobile computing,node distance information,optimization,Optimization methods,position estimation,position estimation.,uniform networks,Vehicles,Wireless sensor networks},
  pages = {961-974},
  file = {/Users/e1727/Dropbox/papers/storage/Localization from connectivity in sensor networks.pdf}
}

@article{Rekleitis2004particle,
  title = {A {{Particle Filter Tutorial}} for {{Mobile Robot Localization}}},
  journal = {Centre for Intelligent Machines, McGill University, Tech. Rep. TR-CIM-04-02},
  author = {Rekleitis, Ioannis M},
  year = {2004},
  file = {/Users/e1727/Dropbox/papers/storage/A particle filter tutorial for mobile robot localization.pdf}
}

@inproceedings{Azuma2013Performance,
  title = {Performance {{Analysis}} of {{Chemotaxis Controllers}}},
  booktitle = {Decision and {{Control}} ({{CDC}}), 2013 {{IEEE}} 52nd {{Annual Conference}} On},
  author = {Azuma, Shun-ichi and Owaki, Katsuya and Shinohara, Nobuhiro and Sugie, Toshiharu},
  year = {2013},
  pages = {1411-1416},
  file = {/Users/e1727/Dropbox/papers/storage/Azuma et al_2013_Performance Analysis of Chemotaxis Controllers2.pdf},
  organization = {IEEE}
}

@inproceedings{Biaz2005Precise,
  title = {Precise {{Distributed Localization Algorithms}} for {{Wireless Networks}}},
  booktitle = {Sixth {{IEEE International Symposium}} on a {{World}} of {{Wireless Mobile}} and {{Multimedia Networks}}},
  doi = {10.1109/WOWMOM.2005.80},
  author = {Biaz, S. and Ji, Yiming},
  month = jun,
  year = {2005},
  keywords = {Multidimensional systems,Network topology,ad hoc networks,estimation error,Estimation error,indoor applications,indoor radio,Iterative algorithms,iterative methods,iterative multidimensional scaling,lateration algorithm,Measurement errors,node position estimation,parameter estimation,precise distributed localization algorithms,Radio communication,radio communication constraints,radio transmission range estimation,range measurement errors,simulated annealing,Simulated annealing,simulated annealing multidimensional scaling,Telecommunication network reliability,telecommunication network topology,Testing,topology randomness,wireless networks,Wireless networks},
  pages = {388-394},
  file = {/Users/e1727/Dropbox/papers/storage/Precise Distributed Localization Algorithms for Wireless Network.pdf},
  note = {ISSN:}
}

@inproceedings{Ranjbar-Sahraei2012Multirobot,
  address = {{Berlin, Heidelberg}},
  title = {A {{Multi}}-Robot {{Coverage Approach Based}} on {{Stigmergic Communication}}},
  isbn = {978-3-642-33690-4},
  abstract = {Recent years have witnessed a rapidly growing interest in using teams of mobile robots for autonomously covering environments. In this paper a novel approach for multi-robot coverage is described which is based on the principle of pheromone-based communication. According to this approach, called StiCo (for ``Stigmergic Coverage''), the robots communicate indirectly via depositing/detecting markers in the environment to be covered. Although the movement policies of each robot are very simple, complex and efficient coverage behavior is achieved at the team level. StiCo shows several desirable features such as robustness, scalability and functional extensibility. Two extensions are described, including A-StiCo for dealing with dynamic environments and ID-StiCo for handling intruder detection. These features make StiCo an interesting alternative to graph-based multi-robot coverage approaches which currently are dominant in the field. Moreover, because of these features StiCo has a broad application potential. Simulation results are shown which clearly demonstrate the strong coverage abilities of StiCo in different environmental settings.},
  booktitle = {Multiagent {{System Technologies}}},
  publisher = {{Springer Berlin Heidelberg}},
  author = {{Ranjbar-Sahraei}, Bijan and Weiss, Gerhard and Nakisaee, Ali},
  editor = {Timm, Ingo J. and Guttmann, Christian},
  year = {2012},
  pages = {126-138},
  file = {/Users/e1727/Dropbox/papers/storage/A Multi-robot Coverage Approach Based on Stigmergic Communication.pdf}
}

@inproceedings{Eren2004Rigidity,
  title = {Rigidity, {{Computation}}, and {{Randomization}} in {{Network Localization}}},
  volume = {4},
  booktitle = {{{IEEE INFOCOM}} 2004},
  doi = {10.1109/INFCOM.2004.1354686},
  author = {Eren, T. and Goldenberg, O. K. and Whiteley, W. and Yang, Y. R. and Morse, A. S. and Anderson, B. D. O. and Belhumeur, P. N.},
  month = mar,
  year = {2004},
  keywords = {network localization,Global Positioning System,Intelligent networks,Testing,computational complexity,Computational complexity,Computer networks,Computer vision,Design engineering,graph rigidity theory,graph theory,grounded graph,Pervasive computing,Printers,Satellites,sensor network,sensors},
  pages = {2673-2684 vol.4},
  file = {/Users/e1727/Dropbox/papers/storage/Rigidity, Computation, and Randomization in Network Localization.pdf},
  issn = {0743-166X}
}

@inproceedings{Moore2004Robust,
  address = {{Baltimore, MD, USA}},
  series = {{{SenSys}} '04},
  title = {Robust {{Distributed Network Localization}} with {{Noisy Range Measurements}}},
  isbn = {1-58113-879-2},
  booktitle = {Proceedings of the {{2Nd International Conference}} on {{Embedded Networked Sensor Systems}}},
  publisher = {{ACM}},
  doi = {10.1145/1031495.1031502},
  author = {Moore, David and Leonard, John and Rus, Daniela and Teller, Seth},
  year = {2004},
  keywords = {localization,location-awareness,mobility,pervasive computing,sensor networks,tracking},
  pages = {50-61},
  file = {/Users/e1727/Dropbox/papers/storage/Robust Distributed Network Localization with Noisy Range Measurements.pdf},
  numpages = {12},
  acmid = {1031502}
}

@inproceedings{Rubenstein2009Scalable,
  title = {Scalable {{Self}}-{{Assembly}} and {{Self}}-{{Repair}} in a {{Collective}} of {{Robots}}},
  booktitle = {2009 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}}},
  doi = {10.1109/IROS.2009.5354716},
  author = {Rubenstein, M. and Shen, W. M.},
  month = oct,
  year = {2009},
  keywords = {distributed control,Mobile robots,multi-robot systems,Bridges,Distributed control,distributed control method,distributed robots,Intelligent robots,Proportional control,robotic collective,Robust control,Self-assembly,Shape control,uncontrolled movement,USA Councils,Wheels},
  pages = {1484-1489},
  file = {/Users/e1727/Dropbox/papers/storage/Scalable self-assembly and self-repair in a collective of robots.pdf},
  issn = {2153-0858}
}

@inproceedings{Rubenstein2010Automatic,
  title = {Automatic {{Scalable Size Selection}} for the {{Shape}} of a {{Distributed Robotic Collective}}},
  booktitle = {2010 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}}},
  doi = {10.1109/IROS.2010.5650906},
  author = {Rubenstein, M. and Shen, W. M.},
  month = oct,
  year = {2010},
  keywords = {multi-robot systems,automatic scalable size selection,distributed robotic collective shape,individual robots,S-DASH,shape control},
  pages = {508-513},
  file = {/Users/e1727/Dropbox/papers/storage/Automatic scalable size selection for the shape of a distributed robotic.pdf},
  issn = {2153-0858}
}

@article{Messina2014Selfassembly,
  title = {Self-{{Assembly}} of {{Magnetic Balls}}: {{From Chains}} to {{Tubes}}},
  volume = {89},
  number = {1},
  journal = {Physical Review E},
  author = {Messina, Ren{\'e} and Khalil, Lara Abou and Stankovi{\'c}, Igor},
  year = {2014},
  pages = {011202},
  file = {/Users/e1727/Dropbox/papers/storage/Self-assembly of magnetic balls.pdf},
  publisher = {APS}
}

@article{Barca2013Swarm,
  title = {Swarm {{Robotics Reviewed}}},
  volume = {31},
  number = {3},
  journal = {Robotica},
  doi = {10.1017/S026357471200032X},
  author = {Barca, Jan Carlo and Sekercioglu, Y. Ahmet},
  year = {2013},
  pages = {345--359},
  file = {/Users/e1727/Dropbox/papers/storage/Swarm Robotics Reviewed.pdf},
  publisher = {Cambridge University Press}
}

@inproceedings{Wang2008decentralized,
  title = {A {{Decentralized Control}} for {{Mobile Sensor Network Effective Coverage}}},
  booktitle = {2008 7th {{World Congress}} on {{Intelligent Control}} and {{Automation}}},
  author = {Wang, Hua and Guo, Yi},
  year = {2008},
  pages = {473-478},
  file = {/Users/e1727/Dropbox/papers/storage/Wang_Guo_2008_A Decentralized Control for Mobile Sensor Network Effective Coverage2.pdf},
  organization = {IEEE}
}

@article{DongJunYi2014marutiezientosisutemunoZhiYu,
  title = {マルチエージェントシステムの制御 : {{V}} 被覆制御},
  volume = {58},
  number = {1},
  journal = {システム／制御／情報},
  doi = {10.11509/isciesci.58.1_36},
  author = {東俊一},
  year = {2014},
  pages = {36-44},
  file = {/Users/e1727/Dropbox/papers/storage/マルチエージェントシステムの制御.pdf}
}

@article{DongJunYi2012FenSanZhiYuniyorurobotutomasugemu,
  title = {分散制御によるロボットマスゲーム},
  volume = {25},
  issn = {1342-5668},
  number = {4},
  journal = {システム制御情報学会論文誌},
  doi = {10.5687/iscie.25.94},
  author = {東俊一 and 泉晋作 and 杉江俊治},
  year = {2012},
  pages = {94-100},
  file = {/Users/e1727/Dropbox/papers/storage/分散制御によるロボットマスゲーム.pdf},
  publisher = {一般社団法人 システム制御情報学会}
}

@article{QuanJinZuo2016ShengWusisutemuniokeruQueLuDeZhiYuQi,
  title = {生物システムにおける確率的制御器},
  volume = {60},
  number = {5},
  journal = {システム／制御／情報},
  doi = {10.11509/isciesci.60.5_205},
  author = {泉晋作},
  year = {2016},
  pages = {205-210},
  file = {/Users/e1727/Dropbox/papers/storage/生物システムにおける確率的制御器.pdf;/Users/e1727/Dropbox/Zotero/storage/6W8S7CMS/10.1007%2F978-3-540-78929-1_26.bib}
}

@article{QuanJinZuo2014DaChangJunnoZouHuaXingZhiYuQiniyoruBeiFuZhiYu,
  title = {大腸菌の走化性制御器による被覆制御：実機実験による検証},
  volume = {57},
  journal = {自動制御連合講演会講演論文集},
  doi = {10.11511/jacc.57.0_2098},
  author = {泉晋作 and 東俊一 and 杉江俊治},
  year = {2014},
  pages = {2098-2100},
  file = {/Users/e1727/Dropbox/papers/storage/大腸菌の走化性制御器による被覆制御.pdf}
}

@article{Zhou2015Distributed,
  title = {Distributed {{Locating Algorithm MDS}}-{{MAP}} ({{LF}}) {{Based}} on {{Low}}-{{Frequency Signal}}},
  volume = {12},
  number = {4},
  journal = {Computer Science and Information Systems},
  author = {Zhou, Chunyue and Xu, Tong and Dong, Hairong},
  year = {2015},
  pages = {1289-1305},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed locating algorithm MDS-MAP (LF) based on low-frequency signal.pdf}
}

@inproceedings{Vella2014magnetoelastica,
  title = {The {{Magneto}}-{{Elastica}}: {{From Self}}-{{Buckling}} to {{Self}}-{{Assembly}}},
  volume = {470},
  booktitle = {Proc. {{R}}. {{Soc}}. {{A}}},
  author = {Vella, Dominic and {du Pontavice}, Emmanuel and Hall, Cameron L and Goriely, Alain},
  year = {2014},
  pages = {20130609},
  file = {/Users/e1727/Dropbox/papers/storage/The magneto-elastica.pdf},
  number = {2162},
  organization = {The Royal Society}
}

@inproceedings{Khaldi2016Virtual,
  address = {{Cham}},
  title = {A {{Virtual Viscoelastic Based Aggregation Model}} for {{Self}}-Organization of {{Swarm Robots System}}},
  isbn = {978-3-319-40379-3},
  abstract = {We report a bio-inspired control model to dynamically self-organize a swarm robots system into unplanned patterns emerged through an aggregation method based upon using virtual viscoelastic links among the K-nearby robots. By varying this neighbourhood relationship, virtual viscoelastic links are dynamically created and destroyed between the robots and their sensed neighbours. Based on the equilibrium between these virtual links, the model can distribute the robots at equal angular configurations of the emergent shape being formed. A forward dependent angular motion control is designed to control at which speeds the robots are moving. The model is implemented and tested using the ARGoS simulator where many emerged self-organized configurations are formed showing the effectiveness of the model.},
  booktitle = {Towards {{Autonomous Robotic Systems}}},
  publisher = {{Springer International Publishing}},
  author = {Khaldi, Belkacem and Cherif, Foudil},
  editor = {Alboul, Lyuba and Damian, Dana and Aitken, Jonathan M.},
  year = {2016},
  pages = {202-213},
  file = {/Users/e1727/Dropbox/papers/storage/A Virtual Viscoelastic Based Aggregation Model for Self-organization of Swarm.pdf}
}

@inproceedings{Mesquita2008Optimotaxis,
  address = {{Berlin, Heidelberg}},
  title = {Optimotaxis: {{A Stochastic Multi}}-Agent {{Optimization Procedure}} with {{Point Measurements}}},
  isbn = {978-3-540-78929-1},
  abstract = {We consider the problem of seeking the maximum of a scalar signal using a swarm of autonomous vehicles equipped with sensors that can take point measurements of the signal. Vehicles are not able to measure their current position or to communicate with each other. Our approach induces the vehicles to perform a biased random walk inspired by bacterial chemotaxis and controlled by a stochastic hybrid automaton. With such a controller, it is shown that the positions of the vehicles evolve towards a probability density that is a specified function of the spatial profile of the measured signal, granting higher vehicle densities near the signal maxima.},
  booktitle = {Hybrid {{Systems}}: {{Computation}} and {{Control}}},
  publisher = {{Springer Berlin Heidelberg}},
  author = {Mesquita, Alexandre R. and Hespanha, Jo{\~a}o P. and {\AA}str{\"o}m, Karl},
  editor = {Egerstedt, Magnus and Mishra, Bud},
  year = {2008},
  pages = {358-371},
  file = {/Users/e1727/Dropbox/papers/storage/Optimotaxis.pdf}
}

@inproceedings{Zhang2006Source,
  title = {Source {{Seeking With Nonholonomic Unicycle Without Position Measurement}}---{{Part I}}: {{Tuning}} of {{Forward Velocity}}},
  booktitle = {Proceedings of the 45th {{IEEE Conference}} on {{Decision}} and {{Control}}},
  doi = {10.1109/CDC.2006.377391},
  author = {Zhang, C. and Arnold, D. and Ghods, N. and Siranosian, A. and Krstic, M.},
  month = dec,
  year = {2006},
  keywords = {mobile robots,Mobile robots,aerial vehicles,angular velocity,Angular velocity,angular velocity control,Angular velocity control,autonomous vehicle,control strategies,Convergence,extremum seeking,forward velocity tuning,Frequency,nonholonomic unicycle,optimal control,periodic control,periodic forward-backward movement,Periodic structures,Position measurement,Remotely operated vehicles,scalar signal,signal detection,source seeking,underwater vehicles,Underwater vehicles,vehicles,Velocity measurement},
  pages = {3040-3045},
  file = {/Users/e1727/Dropbox/papers/storage/Source Seeking With Nonholonomic Unicycle Without Position Measurement---Part I.pdf},
  issn = {0191-2216}
}

@article{Bandyopadhyay2017Probabilistic,
  title = {Probabilistic and {{Distributed Control}} of a {{Large}}-{{Scale Swarm}} of {{Autonomous Agents}}},
  volume = {33},
  number = {5},
  journal = {IEEE Transactions on Robotics},
  author = {Bandyopadhyay, Saptarshi and Chung, Soon-Jo and Hadaegh, Fred Y},
  year = {2017},
  pages = {1103-1123},
  file = {/Users/e1727/Dropbox/papers/storage/Probabilistic and distributed control of a large-scale swarm of autonomous.pdf},
  publisher = {IEEE}
}

@incollection{Trawny2010global,
  title = {On the {{Global Optimum}} of {{Planar}}, {{Range}}-{{Based Robot}}-to-{{Robot Relative Pose Estimation}}},
  isbn = {978-1-4244-5038-1},
  abstract = {In this paper, we address the problem of determining the relative position and orientation (pose) of two robots navigating in 2D, based on known egomotion and noisy robot-to-robot distance measurements. We formulate this as a weighted Least Squares (WLS) estimation problem, and determine the exact global optimum by directly solving the multivariate polynomial system resulting from the first-order optimality conditions. Given the poor scalability of the original WLS problem, we propose an alternative formulation of the WLS problem in terms of squared distance measurements (squared distancesWLS or SD-WLS). Using a hybrid algebraic-numeric technique, we are able to solve the corresponding first-order optimality conditions of the SD-WLS in 125 ms in Matlab. Both methods solve the minimal (3 distance measurements) as well as the overdetermined problem (more than 3 measurements) in a unified fashion. Simulation and experimental results show that the SD-WLS achieves performance virtually indistinguishable from the maximum likelihood estimator, and significantly outperforms current algebraic methods.},
  booktitle = {2010 {{IEEE International Conference}} on {{Robotics}} and {{Automation}}, {{ICRA}} 2010},
  author = {Trawny, Nikolas and Roumeliotis, Stergios I.},
  month = aug,
  year = {2010},
  pages = {3200-3206},
  file = {/Users/e1727/Dropbox/papers/storage/On the global optimum of planar, range-based robot-to-robot relative pose.pdf},
  doi = {10.1109/ROBOT.2010.5509541}
}

@article{Zhou2008RobottoRobot,
  title = {Robot-to-{{Robot Relative Pose Estimation From Range Measurements}}},
  volume = {24},
  issn = {1552-3098},
  number = {6},
  journal = {IEEE Transactions on Robotics},
  doi = {10.1109/TRO.2008.2006251},
  author = {Zhou, X. S. and Roumeliotis, S. I.},
  month = dec,
  year = {2008},
  keywords = {distance measurement,Distance measurement,range measurements,robot vision,iterative methods,iterative least-squares process,least mean squares methods,Lie algebras,Lie derivatives,nonlinear control systems,nonsingular configurations,observability conditions,observability of nonlinear systems,pose estimation,relative pose estimation,robot-to-robot distance measurements,robot-to-robot relative pose estimation},
  pages = {1379-1393},
  file = {/Users/e1727/Dropbox/papers/storage/Robot-to-Robot Relative Pose Estimation From Range Measurements.pdf}
}

@article{DaZeXiuYi2008sensahuyuziyonniyoruYiDongTinoZiJiWeiZhiTuiDing,
  title = {センサフュージョンによる移動体の自己位置推定},
  volume = {51},
  journal = {自動制御連合講演会講演論文集},
  doi = {10.11511/jacc.51.0.189.0},
  author = {{大澤修一} and {中村文一} and {西谷紘一}},
  year = {2008},
  pages = {189-189},
  file = {/Users/e1727/Dropbox/papers/storage/センサフュージョンによる移動体の自己位置推定.pdf}
}

@book{Nocedal2006Numerical,
  title = {Numerical {{Optimization}}},
  isbn = {978-0-387-30303-1},
  publisher = {{Springer}},
  author = {Nocedal, Jorge},
  year = {2006}
}

@article{Petersen2012Matrix,
  title = {The {{Matrix Cookbook}}},
  abstract = {Matrix identities, relations and approximations. A desktop reference for quick overview of mathematics of matrices.},
  author = {Petersen, K. B. and Pedersen, M. S.},
  month = nov,
  year = {2012},
  keywords = {inverse,matrix derivative,Matrix identity,matrix relations},
  file = {/Users/e1727/Dropbox/papers/storage/The Matrix Cookbook.pdf},
  publisher = {Technical University of Denmark},
  note = {Version 20121115}
}

@article{Pimenta2013Swarm,
  title = {Swarm {{Coordination Based}} on {{Smoothed Particle Hydrodynamics Technique}}},
  volume = {29},
  issn = {1552-3098},
  number = {2},
  journal = {IEEE Transactions on Robotics},
  doi = {10.1109/TRO.2012.2234294},
  author = {Pimenta, L. C. A. and Pereira, G. A. S. and Michael, N. and Mesquita, R. C. and Bosque, M. M. and Chaimowicz, L. and Kumar, V.},
  month = apr,
  year = {2013},
  keywords = {Equations,motion control,multi-robot systems,Robot kinematics,computer simulations,convergence,decentralized controllers,Distributed robot systems,dynamic obstacles,feedback,feedback control laws,finite size constraints,fluid dynamics,fluid particles,Harmonic analysis,hazardous areas,hydrodynamics,Hydrodynamics,incompressible fluid model,Kernel,Mathematical model,nonholonomic constraints,pattern generation task,robot swarms,smoothed particle hydrodynamics (SPH),smoothed particle hydrodynamics technique,smoothed-particle hydrodynamics,SPH method,SPH technique,stability,static obstacles,swarm coordination,swarm robotics},
  pages = {383-399},
  file = {/Users/e1727/Dropbox/papers/storage/Swarm Coordination Based on Smoothed Particle Hydrodynamics Technique.pdf}
}

@inproceedings{Calafiore2010Distributed,
  title = {Distributed {{Optimization Techniques}} for {{Range Localization}} in {{Networked Systems}}},
  booktitle = {49th {{IEEE Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  doi = {10.1109/CDC.2010.5717645},
  author = {Calafiore, G. C. and Carlone, L. and Wei, M.},
  month = dec,
  year = {2010},
  keywords = {agents measurements,agents position,Barzilai-Borwein stepsizes,consensus,distance measurement,Distance measurement,Distributed algorithms,distributed control,distributed estimation,distributed Gauss-Newton approach,distributed gradient method,distributed optimization,distributed optimization techniques,Equations,estimation theory,gradient methods,Gradient methods,mobile agents,network connectivity,network localization,Network localization,networked systems,optimisation,pairwise distance measurements,range localization,range measurements,Robot sensing systems,state-of-the-art algorithms,Symmetric matrices,telecommunication control,wireless sensor networks},
  pages = {2221-2226},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed Optimization Techniques for Range Localization in Networked Systems.pdf},
  issn = {0191-2216}
}

@book{PianShanChe2000YingYongkarumanhuiruta,
  title = {応用カルマンフィルタ},
  isbn = {4-254-20101-X},
  publisher = {{朝倉書店}},
  author = {片山徹},
  year = {2000}
}

@inproceedings{Martinelli2005MultiRobot,
  title = {Multi-{{Robot Localization Using Relative Observations}}},
  booktitle = {Proceedings of the 2005 {{IEEE International Conference}} on {{Robotics}} and {{Automation}}},
  doi = {10.1109/ROBOT.2005.1570537},
  author = {Martinelli, A. and Pont, F. and Siegwart, R.},
  month = apr,
  year = {2005},
  keywords = {Equations,Robot sensing systems,Mobile robots,Collaboration,Filters,Fuses,Kalman filter,Monitoring,Multi-Robot Localization,Navigation,Relative Observation,Robot localization,Robot Navigation,Sensor fusion,Sensor Fusion},
  pages = {2797-2802},
  file = {/Users/e1727/Dropbox/papers/storage/Multi-robot localization using relative observations.pdf},
  issn = {1050-4729}
}

@inproceedings{Mao2007Design,
  title = {Design of an {{Extended Kalman Filter}} for {{UAV Localization}}},
  booktitle = {2007 {{Information}}, {{Decision}} and {{Control}}},
  doi = {10.1109/IDC.2007.374554},
  author = {Mao, G. and Drake, S. and Anderson, B. D. O.},
  month = feb,
  year = {2007},
  keywords = {Distance measurement,Global Positioning System,Design engineering,Navigation,aerospace control,Australia,Automotive engineering,Control design,extended Kalman filter,GPS signal,Interference,interUAV distance measurement,Loss measurement,navigation,nonlinear filters,remotely operated vehicles,UAV localization,unmanned aerial vehicle,Unmanned aerial vehicles},
  pages = {224-229},
  file = {/Users/e1727/Dropbox/papers/storage/Design of an Extended Kalman Filter for UAV Localization.pdf}
}

@article{Roumeliotis2002Distributed,
  title = {Distributed {{Multirobot Localization}}},
  volume = {18},
  issn = {1042-296X},
  number = {5},
  journal = {IEEE Transactions on Robotics and Automation},
  doi = {10.1109/TRA.2002.803461},
  author = {Roumeliotis, S. I. and Bekey, G. A.},
  month = oct,
  year = {2002},
  keywords = {Robot sensing systems,mobile robots,Mobile robots,Computer science,decentralised control,multi-robot systems,Robot kinematics,Kalman filter,Area measurement,collective localization,decentralized estimation,decentralized information filter,distributed multiple robot localization,Information filtering,Information filters,Kalman filters,Magnetic field measurement,Magnetic sensors,observability,position control,positioning,sensor data acquisition,sensor fusion,Working environment noise},
  pages = {781-795},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed multirobot localization.pdf}
}

@article{Xunaue2008Distributed,
  title = {Distributed {{Localization}} for {{Anchor}}-{{Free Sensor Networks}}},
  volume = {19},
  number = {3},
  journal = {Journal of Systems Engineering and Electronics},
  doi = {10.1016/S1004-4132(08)60100-0},
  author = {Xunaue, C. and Zhiguan, S. and Jianjun, L.},
  month = jun,
  year = {2008},
  keywords = {Distance measurement,position estimation,sensor networks,anchor-free localization,Current measurement,distributed algorithm,Force,Layout,Optimization,Reliability,Springs},
  pages = {405-418},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed localization for anchor-free sensor networks.pdf}
}

@inproceedings{Viegas2012Decentralized,
  title = {Decentralized {{Range}}-{{Based Linear Motion Estimation}} in {{Acyclic Vehicle Formations}} with {{Fixed Topologies}}},
  booktitle = {2012 {{American Control Conference}} ({{ACC}})},
  doi = {10.1109/ACC.2012.6314915},
  author = {Viegas, D. and Batista, P. and Oliveira, P. and Silvestre, C.},
  month = jun,
  year = {2012},
  keywords = {mobile robots,motion control,motion estimation,decentralised control,multi-robot systems,graph theory,Position measurement,vehicles,Velocity measurement,acyclic graph,acyclic vehicle formations,asymptotic stability,autonomous vehicles,decentralized range-based linear motion estimation,decentralized state estimation,fixed topologies,globally exponentially stable error dynamics,Noise measurement,Nonlinear dynamical systems,Observability,Observers,state estimation},
  pages = {6575-6580},
  file = {/Users/e1727/Dropbox/papers/storage/Decentralized range-based linear motion estimation in acyclic vehicle.pdf},
  issn = {0743-1619}
}

@inproceedings{Panzieri2006Multirobot,
  title = {Multirobot {{Localisation Using Interlaced Extended Kalman Filter}}},
  booktitle = {2006 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}}},
  doi = {10.1109/IROS.2006.282065},
  author = {Panzieri, S. and Pascucci, F. and Setola, R.},
  month = oct,
  year = {2006},
  keywords = {Robot sensing systems,Mobile robots,decentralised control,multi-robot systems,sensors,Intelligent robots,Navigation,Robot localization,Kalman filters,Collaborative work,data exchange,decentralized algorithm,distribuited Kalman filter,interlaced extended Kalman filter,multirobot localisation,Multirobot localization,Particle filters,path planning,Robustness,Security,Wireless communication,wireless communication devices},
  pages = {2816-2821},
  file = {/Users/e1727/Dropbox/papers/storage/Multirobot Localisation Using Interlaced Extended Kalman Filter.pdf},
  issn = {2153-0858}
}

@article{Choi2011Hierarchical,
  title = {A {{Hierarchical Algorithm}} for {{Indoor Mobile Robot Localization Using RFID Sensor Fusion}}},
  volume = {58},
  issn = {0278-0046},
  number = {6},
  journal = {IEEE Transactions on Industrial Electronics},
  doi = {10.1109/TIE.2011.2109330},
  author = {Choi, B. S. and Lee, J. W. and Lee, J. J. and Park, K. T.},
  month = jun,
  year = {2011},
  keywords = {Robot sensing systems,mobile robots,Mobile robots,position control,sensor fusion,Acoustics,distance data,global position estimation,GPE process,hierarchical localization algorithm,indoor mobile robot localization,LEC process,local environment cognition,Localization,mobile robot,obstacle estimation,radio-frequency identification,radio-frequency identification (RFID),radiofrequency identification,RFID sensor fusion,RFID tag,RFID tags,RFID-based mobile robot localization,stand-alone RFID system,ultrasonic sensor system,ultrasonic transducers,Uncertainty},
  pages = {2226-2235},
  file = {/Users/e1727/Dropbox/papers/storage/A Hierarchical Algorithm for Indoor Mobile Robot Localization Using RFID Sensor.pdf}
}

@article{La2013Distributed,
  title = {Distributed {{Sensor Fusion}} for {{Scalar Field Mapping Using Mobile Sensor Networks}}},
  volume = {43},
  issn = {2168-2267},
  number = {2},
  journal = {IEEE Transactions on Cybernetics},
  doi = {10.1109/TSMCB.2012.2215919},
  author = {La, H. M. and Sheng, W.},
  month = apr,
  year = {2013},
  keywords = {Sensor fusion,sensor fusion,Algorithm design and analysis,autonomous mobile sensor networks,Cooperative sensing,distributed consensus filter,distributed flocking-control algorithm,distributed sensor fusion algorithm,Estimation,flocking control,Heuristic algorithms,iterative method,Mobile communication,mobile radio,mobile sensor networks (MSNs),noisy sensor measurements,scalar field mapping,Time measurement,weighted average consensus filter},
  pages = {766-778},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed Sensor Fusion for Scalar Field Mapping Using Mobile Sensor Networks.pdf}
}

@inproceedings{Deming2005Sensor,
  title = {Sensor {{Fusion}} for {{Swarms}} of {{Unmanned Aerial Vehicles Using Modeling Field Theory}}},
  booktitle = {International {{Conference}} on {{Integration}} of {{Knowledge Intensive Multi}}-{{Agent Systems}}, 2005.},
  doi = {10.1109/KIMAS.2005.1427065},
  author = {Deming, R.},
  month = apr,
  year = {2005},
  keywords = {Collision avoidance,Sensor fusion,remotely operated vehicles,Unmanned aerial vehicles,sensor fusion,aircraft control,automatic collision avoidance,Automatic control,automatic target detection,autonomous operation,collision avoidance,combinatorial complexity,Force measurement,fuzzy dynamic logic,fuzzy logic,Humans,image interpretation,image representation,Image sensors,Intelligent sensors,modeling field theory,Object detection,Performance evaluation,target discrimination,target localization,target tracking,UAV control,UAV track,unmanned aerial vehicle swarm,visual sensor},
  pages = {122-127}
}

@book{Boyd2004Convex,
  title = {Convex Optimization},
  isbn = {978-0-521-83378-3},
  publisher = {{Cambridge University Press}},
  author = {Boyd, Stephen},
  year = {2004}
}

@inproceedings{Hsieh2006Pattern,
  title = {Pattern Generation with Multiple Robots},
  booktitle = {Proceedings 2006 {{IEEE International Conference}} on {{Robotics}} and {{Automation}}, 2006. {{ICRA}} 2006.},
  doi = {10.1109/ROBOT.2006.1642068},
  author = {Hsieh, Mong-ying A. and Kumar, V.},
  month = may,
  year = {2006},
  keywords = {Robot sensing systems,decentralised control,multi-robot systems,Robot kinematics,Shape control,Convergence,convergence,stability,Biology computing,Communication system control,decentralized control,multiple robots,pattern generation,range sensors,Sensor phenomena and characterization,Stability,Surveillance,Topology,two-dimensional geometric pattern},
  pages = {2442-2447},
  file = {/Users/e1727/Dropbox/papers/storage/Pattern generation with multiple robots.pdf},
  issn = {1050-4729}
}

@article{MorrisSimulating,
  title = {Simulating Surface Tension with Smoothed Particle Hydrodynamics},
  volume = {33},
  abstract = {Abstract A method for simulating two-phase flows including surface tension is presented. The approach is based upon smoothed particle hydrodynamics (SPH). The fully Lagrangian nature of SPH maintains sharp fluid\textendash{}fluid interfaces without employing high-order advection schemes or explicit interface reconstruction. Several possible implementations of surface tension force are suggested and compared. The numerical stability of the method is investigated and optimal choices for numerical parameters are identified. Comparisons with a grid-based volume of fluid method for two-dimensional flows are excellent. The methods presented here apply to problems involving interfaces of arbitrary shape undergoing fragmentation and coalescence within a two-phase system and readily extend to three-dimensional problems. Boundary conditions at a solid surface, high viscosity and density ratios, and the simulation of free-surface flows are not addressed. Copyright \textcopyright{} 2000 John Wiley \& Sons, Ltd.},
  number = {3},
  journal = {International Journal for Numerical Methods in Fluids},
  doi = {10.1002/1097-0363(20000615)33:3<333::AID-FLD11>3.0.CO;2-7},
  author = {Morris, Joseph P.},
  keywords = {interfacial flow,meshless methods,surface tension},
  pages = {333-353},
  file = {/Users/e1727/Dropbox/papers/storage/Simulating surface tension with smoothed particle hydrodynamics.pdf}
}

@inproceedings{St-Pierre2004Comparison,
  title = {Comparison between the Unscented {{Kalman}} Filter and the Extended {{Kalman}} Filter for the Position Estimation Module of an Integrated Navigation Information System},
  booktitle = {{{IEEE Intelligent Vehicles Symposium}}, 2004},
  doi = {10.1109/IVS.2004.1336492},
  author = {{St-Pierre}, M. and Gingras, D.},
  month = jun,
  year = {2004},
  keywords = {Computer science,Global Positioning System,Vehicles,Position measurement,Navigation,Sensor fusion,extended Kalman filter,Kalman filters,sensor fusion,automobiles,car,data fusion method,driver information systems,Electrical engineering,empirical analysis,filtering theory,Gaussian noise,Information systems,integrated navigation information system,Monte Carlo methods,performance evaluation,position estimation module,positioning problems,unscented Kalman filter},
  pages = {831--835},
  file = {/Users/e1727/Dropbox/papers/storage/Comparison between the unscented Kalman filter and the extended Kalman filter.pdf}
}

@article{Stroock1974stochastic,
  title = {Some {{Stochastic Processes Which Arise}} from a {{Model}} of the {{Motion}} of a {{Bacterium}}},
  volume = {28},
  issn = {1432-2064},
  number = {4},
  journal = {Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und Verwandte Gebiete},
  doi = {10.1007/BF00532948},
  author = {Stroock, Daniel W.},
  year = {1974},
  pages = {305-315},
  file = {/Users/e1727/Dropbox/papers/storage/Some stochastic processes which arise from a model of the motion of a bacterium.pdf}
}

@article{Liu2015Dissipative,
  title = {Dissipative {{Particle Dynamics}} ({{DPD}}): {{An Overview}} and {{Recent Developments}}},
  volume = {22},
  issn = {1886-1784},
  abstract = {Dissipative particle dynamics (DPD) is a mesoscale particle method that bridges the gap between microscopic and macroscopic simulations. It can be regarded as a coarse-grained molecular dynamics method suitable for larger time and length scales. It has been successfully applied to different areas of interests, especially in modeling the hydrodynamic behavior of complex fluids in mesoscale. This paper presents an overview on DPD including the methodology, formulation, implementation procedure and some related numerical aspects. The paper also reviews the major applications of the DPD method, especially in modeling (1) micro drop dynamics, (2) multiphase flows in micro-channels and fracture networks, (3) movement and suspension of macromolecules in micro channels and (4) movement and deformation of single cells. The paper ends with some concluding remarks summarizing the major features and future possible development of this unique mesoscale modeling technique.},
  number = {4},
  journal = {Archives of Computational Methods in Engineering},
  doi = {10.1007/s11831-014-9124-x},
  author = {Liu, M. B. and Liu, G. R. and Zhou, L. W. and Chang, J. Z.},
  month = nov,
  year = {2015},
  pages = {529-556},
  file = {/Users/e1727/Dropbox/papers/storage/Dissipative Particle Dynamics (DPD).pdf},
  day = {01}
}

@article{Czirok1999Collective,
  title = {Collective {{Motion}} of {{Self}}-{{Propelled Particles}}: {{Kinetic Phase Transition}} in {{One Dimension}}},
  volume = {82},
  number = {1},
  journal = {Physical Review Letters},
  author = {Czir{\'o}k, Andr{\'a}s and Barab{\'a}si, Albert-L{\'a}szl{\'o} and Vicsek, Tam{\'a}s},
  year = {1999},
  pages = {209},
  publisher = {APS}
}

@article{Czirok2000Collective,
  title = {Collective {{Behavior}} of {{Interacting Self}}-{{Propelled Particles}}},
  volume = {281},
  number = {1-4},
  journal = {Physica A: Statistical Mechanics and its Applications},
  author = {Czir{\'o}k, Andr{\'a}s and Vicsek, Tam{\'a}s},
  year = {2000},
  pages = {17-29},
  file = {/Users/e1727/Dropbox/papers/storage/Czirók_Vicsek_2000_Collective Behavior of Interacting Self-Propelled Particles.pdf},
  publisher = {Elsevier}
}

@article{Vicsek1995Novel,
  title = {Novel {{Type}} of {{Phase Transition}} in a {{System}} of {{Self}}-{{Driven Particles}}},
  volume = {75},
  number = {6},
  journal = {Physical review letters},
  author = {Vicsek, Tam{\'a}s and Czir{\'o}k, Andr{\'a}s and {Ben-Jacob}, Eshel and Cohen, Inon and Shochet, Ofer},
  year = {1995},
  pages = {1226},
  file = {/Users/e1727/Dropbox/papers/storage/Novel type of phase transition in a system of self-driven particles.pdf},
  publisher = {APS}
}

@article{Csahok1998Hydrodynamics,
  title = {Hydrodynamics of {{Bacterial Motion}}},
  journal = {arXiv preprint cond-mat/9811247},
  author = {Csah{\'o}k, Zolt{\'a}n and Czir{\'o}k, Andr{\'a}s},
  year = {1998}
}

@article{DaDou2013JinBangnorobotutotoZhangHaiWunoShiBiewoBiYaotosinaiYiDongrobotutoQunnoZhiYuarugorizumu,
  title = {近傍のロボットと障害物の識別を必要としない移動ロボット群の制御アルゴリズム},
  volume = {49},
  number = {8},
  journal = {計測自動制御学会論文集},
  doi = {10.9746/sicetr.49.787},
  author = {大斗, 坂井 and 宏明, 福島 and 文俊, 松野},
  year = {2013},
  pages = {787-794},
  file = {/Users/e1727/Dropbox/papers/storage/近傍のロボットと障害物の識別を必要としない移動ロボット群の制御アルゴリズム.pdf}
}

@article{DinoueDistributed2018,
  title = {群ロボットシステムの分散自己位置推定},
  journal = {豊田中央研究所研究報告書},
  author = {井上大輔},
  year = {2018},
  pages = {201804007}
}

@article{Izumi2015Distributed,
  title = {Distributed {{Hybrid Controllers}} for {{Multi}}-{{Agent Mass Games By A Variable Number}} of {{Player Agents}}},
  volume = {17},
  abstract = {AbstractThis paper considers a problem of finding distributed controllers for the multi-agent mass games, that is, to let agents organize themselves into a formation displaying a given grayscale image. As a solution to this problem, we propose distributed hybrid controllers. The key idea is to combine a coverage control method and halftone image processing, i.e., to combine techniques from the control theory and the image processing. The performance of the proposed controllers is demonstrated by numerical experiments with standard images.\textcopyright{} 2014 Chinese Automatic Control Society and Wiley Publishing Asia Pty Ltd},
  number = {3},
  journal = {Asian Journal of Control},
  doi = {10.1002/asjc.930},
  author = {Izumi, Shinsaku and Azuma, Shunichi and Sugie, Toshiharu},
  year = {2015},
  keywords = {distributed control,halftone image processing,Multi‐agent system},
  pages = {762-774},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed Hybrid Controllers for Multi‐Agent Mass Games By A Variable Number.pdf},
  eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/asjc.930}
}

@article{Chaurasiya2014novel,
  title = {A {{Novel Distance Estimation Approach}} for 3d {{Localization}} in {{Wireless Sensor Network Using Multi Dimensional Scaling}}},
  volume = {15},
  journal = {Information Fusion},
  author = {Chaurasiya, Vijay K and Jain, Neeraj and Nandi, Gora Chand},
  year = {2014},
  pages = {5-18},
  file = {/Users/e1727/Dropbox/papers/storage/A novel distance estimation approach for 3D localization in wireless sensor.pdf},
  publisher = {Elsevier}
}

@article{Chan2009novel,
  title = {A {{Novel Subspace Approach}} for {{Cooperative Localization}} in {{Wireless Sensor Networks Using Range Measurements}}},
  volume = {57},
  number = {1},
  journal = {IEEE Transactions on Signal Processing},
  author = {Chan, Frankie KW and So, Hing-Cheung and Ma, W-K},
  year = {2009},
  pages = {260-269},
  file = {/Users/e1727/Dropbox/papers/storage/A novel subspace approach for cooperative localization in wireless sensor.pdf},
  publisher = {IEEE}
}

@article{Khan2010DILAND,
  title = {{{DILAND}}: {{An}} Algorithm for Distributed Sensor Localization with Noisy Distance Measurements},
  volume = {58},
  number = {3},
  journal = {IEEE Transactions on Signal Processing},
  author = {Khan, Usman A and Kar, Soummya and Moura, Jos{\'e} MF},
  year = {2010},
  pages = {1940-1947},
  file = {/Users/e1727/Dropbox/papers/storage/DILAND.pdf},
  publisher = {IEEE}
}

@inproceedings{Dil2006Rangebased,
  title = {Range-{{Based Localization}} in {{Mobile Sensor Networks}}},
  booktitle = {European {{Workshop}} on {{Wireless Sensor Networks}}},
  author = {Dil, Bram and Dulman, Stefan and Havinga, Paul},
  year = {2006},
  pages = {164-179},
  file = {/Users/e1727/Dropbox/papers/storage/Range-Based Localization in Mobile Sensor Networks.pdf},
  organization = {Springer}
}

@article{Biswas2006Semidefinite,
  title = {Semidefinite {{Programming Approaches}} for {{Sensor Network Localization}} with {{Noisy Distance Measurements}}},
  volume = {3},
  number = {4},
  journal = {IEEE transactions on automation science and engineering},
  author = {Biswas, Pratik and Liang, T-C and Toh, K-C and Ye, Yinyu and Wang, T-C},
  year = {2006},
  pages = {360-371},
  file = {/Users/e1727/Dropbox/papers/storage/Semidefinite programming approaches for sensor network localization with noisy.pdf},
  publisher = {IEEE}
}

@article{Soares2015Simple,
  title = {Simple and {{Fast Convex Relaxation Method}} for {{Cooperative Localization}} in {{Sensor Networks Using Range Measurements}}},
  volume = {63},
  issn = {1053-587X},
  number = {17},
  journal = {IEEE Transactions on Signal Processing},
  doi = {10.1109/TSP.2015.2454853},
  author = {Soares, C. and Xavier, J. and Gomes, J.},
  month = sep,
  year = {2015},
  keywords = {gradient methods,Robot sensing systems,wireless sensor networks,Convergence,Optimization,Noise measurement,Complexity theory,concave programming,convergence method,convergence of numerical methods,convex programming,convex relaxation method,Convex relaxations,cooperative communication,cooperative localization,distributed algorithms,distributed iterative sensor localization,iteration complexity analysis,maximum likelihood estimation,Maximum likelihood estimation,noisy range measurement,nonconvex maximum likelihood formulation,nonconvex optimization,optimal gradient method,optimization properties,relaxation theory,sensor placement,Signal processing algorithms,wireless sensor network localization problem},
  pages = {4532-4543},
  file = {/Users/e1727/Dropbox/papers/storage/Simple and Fast Convex Relaxation Method for Cooperative Localization in Sensor.pdf}
}

@book{Tan2015Handbook,
  address = {{Hershey, PA, USA}},
  edition = {1st},
  title = {Handbook of {{Research}} on {{Design}}, {{Control}}, and {{Modeling}} of {{Swarm Robotics}}},
  isbn = {1-4666-9572-2 978-1-4666-9572-6},
  publisher = {{IGI Global}},
  author = {Tan, Ying},
  year = {2015}
}

@article{Chavanis2008Nonlinear,
  title = {Nonlinear {{Mean Field Fokker}}-{{Planck Equations}}. {{Application}} to the {{Chemotaxis}} of {{Biological Populations}}},
  volume = {62},
  number = {2},
  journal = {The European Physical Journal B},
  author = {Chavanis, Pierre-Henri},
  year = {2008},
  pages = {179-208},
  file = {/Users/e1727/Dropbox/papers/storage/Nonlinear Mean Field Fokker-Planck Equations.pdf},
  publisher = {Springer}
}

@article{Shiino2003Stability,
  title = {Stability {{Analysis}} of {{Mean}}-{{Field}}-{{Type Nonlinear Fokker}}-{{Planck Equations Associated}} with a {{Generalized Entropy}} and {{Its Application}} to the {{Self}}-{{Gravitating System}}},
  volume = {67},
  number = {5},
  journal = {Physical Review E},
  author = {Shiino, Masatoshi},
  year = {2003},
  pages = {056118},
  file = {/Users/e1727/Dropbox/papers/storage/Stability analysis of mean-field-type nonlinear Fokker-Planck equations.pdf},
  publisher = {APS}
}

@article{Horsthemke1977Meanfield,
  title = {Mean-{{Field Theory}} of {{Critical Behaviour}} and {{First Order Transition}}: {{A Comparison Between}} the {{Master Equation}} and the {{Nonlinear Fokker}}-{{Planck Equation}}},
  volume = {28},
  number = {2},
  journal = {Zeitschrift f{\"u}r Physik B Condensed Matter},
  author = {Horsthemke, Werner and {Malek-Mansour}, M and Brenig, L{\'e}on},
  year = {1977},
  pages = {135-139},
  file = {/Users/e1727/Dropbox/papers/storage/Mean-field theory of critical behaviour and first order transition.pdf},
  publisher = {Springer}
}

@article{Chavanis2006Nonlinear,
  title = {Nonlinear {{Mean}}-{{Field Fokker}}-{{Planck Equations}} and {{Their Applications}} in {{Physics}}, {{Astrophysics}} and {{Biology}}},
  journal = {arXiv preprint cond-mat/0611087},
  author = {Chavanis, Pierre-Henri},
  year = {2006},
  file = {/Users/e1727/Dropbox/papers/storage/Nonlinear Mean-Field Fokker-Planck Equations and Their Applications in Physics,.pdf}
}

@article{Martzel2001Meanfield,
  title = {Mean-{{Field Treatment}} of the {{Many}}-{{Body Fokker}}--{{Planck Equation}}},
  volume = {34},
  number = {50},
  journal = {Journal of Physics A: Mathematical and General},
  author = {Martzel, Nicolas and Aslangul, Claude},
  year = {2001},
  pages = {11225},
  file = {/Users/e1727/Dropbox/papers/storage/Mean-field treatment of the many-body Fokker--Planck equation.pdf},
  publisher = {IOP Publishing}
}

@article{Cao1997Cooperative,
  title = {Cooperative {{Mobile Robotics}}: {{Antecedents}} and {{Directions}}},
  volume = {4},
  number = {1},
  journal = {Autonomous robots},
  author = {Cao, Y Uny and Fukunaga, Alex S and Kahng, Andrew},
  year = {1997},
  pages = {7-27},
  publisher = {Springer}
}

@article{Brambilla2013Swarm,
  title = {Swarm {{Robotics}}: {{A Review}} from the {{Swarm Engineering Perspective}}},
  volume = {7},
  number = {1},
  journal = {Swarm Intelligence},
  author = {Brambilla, Manuele and Ferrante, Eliseo and Birattari, Mauro and Dorigo, Marco},
  year = {2013},
  pages = {1-41},
  publisher = {Springer}
}

@inproceedings{Sahin2004Swarm,
  title = {Swarm {{Robotics}}: {{From Sources}} of {{Inspiration}} to {{Domains}} of {{Application}}},
  booktitle = {International Workshop on Swarm Robotics},
  author = {Sahin, Erol},
  year = {2004},
  pages = {10-20},
  file = {/Users/e1727/Dropbox/papers/storage/Swarm robotics2.pdf},
  organization = {Springer}
}

@article{Kube2000Cooperative,
  title = {Cooperative {{Transport}} by {{Ants}} and {{Robots}}},
  volume = {30},
  number = {1-2},
  journal = {Robotics and autonomous systems},
  author = {Kube, C Ronald and Bonabeau, Eric},
  year = {2000},
  pages = {85-101},
  file = {/Users/e1727/Dropbox/papers/storage/Cooperative transport by ants and robots.pdf},
  publisher = {Elsevier}
}

@article{Cheah2009Regionbased,
  title = {Region-{{Based Shape Control}} for a {{Swarm}} of {{Robots}}},
  volume = {45},
  number = {10},
  journal = {Automatica},
  author = {Cheah, Chien Chern and Hou, Saing Paul and Slotine, Jean Jacques E},
  year = {2009},
  pages = {2406-2411},
  file = {/Users/e1727/Dropbox/papers/storage/Region-Based Shape Control for a Swarm of Robots.pdf},
  publisher = {Elsevier}
}

@article{Xie2007Consensus,
  title = {Consensus {{Control}} for a {{Class}} of {{Networks}} of {{Dynamic Agents}}},
  volume = {17},
  number = {10-11},
  journal = {International Journal of Robust and Nonlinear Control: IFAC-Affiliated Journal},
  author = {Xie, Guangming and Wang, Long},
  year = {2007},
  pages = {941-959},
  publisher = {Wiley Online Library}
}

@article{Spears2004Distributed,
  title = {Distributed, {{Physics}}-{{Based Control}} of {{Swarms}} of {{Vehicles}}},
  volume = {17},
  number = {2-3},
  journal = {Autonomous Robots},
  author = {Spears, William M and Spears, Diana F and Hamann, Jerry C and Heil, Rodney},
  year = {2004},
  pages = {137-162},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed, physics-based control of swarms of vehicles.pdf},
  publisher = {Springer}
}

@article{Castillo2012Comparative,
  title = {Comparative {{Study}} of {{Bio}}-{{Inspired Algorithms Applied}} to the {{Optimization}} of {{Type}}-1 and {{Type}}-2 {{Fuzzy Controllers}} for an {{Autonomous Mobile Robot}}},
  volume = {192},
  journal = {Information sciences},
  author = {Castillo, Oscar and {Mart{\'i}nez-Marroqu{\'i}n}, Ricardo and Melin, Patricia and Valdez, Fevrier and Soria, Jos{\'e}},
  year = {2012},
  pages = {19-38},
  publisher = {Elsevier}
}

@incollection{Kourogi2006Indoor,
  title = {Indoor/Outdoor Pedestrian Navigation with an Embedded {{GPS}}/{{RFID}}/Self-Contained Sensor System},
  booktitle = {Advances in {{Artificial Reality}} and {{Tele}}-{{Existence}}},
  publisher = {{Springer}},
  author = {Kourogi, Masakatsu and Sakata, Nobuchika and Okuma, Takashi and Kurata, Takeshi},
  year = {2006},
  pages = {1310-1321},
  file = {/Users/e1727/Dropbox/papers/storage/Indoor-outdoor pedestrian navigation with an embedded GPS-RFID-self-contained.pdf;/Users/e1727/Dropbox/Zotero/storage/NUW7P5DD/10.1007%2F978-3-540-78929-1_26.bib}
}

@article{Luo2014Multiple,
  title = {Multiple {{Object Tracking}}: {{A Review}}},
  volume = {1},
  journal = {arXiv preprint arXiv:1409.7618},
  author = {Luo, Wenhan and Zhao, Xiaowei and Kim, Tae-Kyun},
  year = {2014},
  file = {/Users/e1727/Dropbox/papers/storage/Multiple object tracking.pdf},
  publisher = {Citeseer}
}

@article{Blais2004Review,
  title = {Review of 20 {{Years}} of {{Range Sensor Development}}},
  volume = {13},
  number = {1},
  journal = {Journal of electronic imaging},
  author = {Blais, Fran{\c c}ois},
  year = {2004},
  pages = {231-244},
  publisher = {International Society for Optics and Photonics}
}

@book{Gustafsson2010Statistical,
  title = {Statistical {{Sensor Fusion}}},
  publisher = {{Studentlitteratur}},
  author = {Gustafsson, Fredrik},
  year = {2010}
}

@article{Cao2006Sensor,
  title = {Sensor {{Network Localization}} with {{Imprecise Distances}}},
  volume = {55},
  number = {11},
  journal = {Systems \& control letters},
  author = {Cao, Ming and Anderson, Brian DO and Morse, A Stephen},
  year = {2006},
  pages = {887-893},
  publisher = {Elsevier}
}

@article{Aspnes2006theory,
  title = {A {{Theory}} of {{Network Localization}}},
  volume = {5},
  number = {12},
  journal = {IEEE Transactions on Mobile Computing},
  author = {Aspnes, James and Eren, Tolga and Goldenberg, David Kiyoshi and Morse, A Stephen and Whiteley, Walter and Yang, Yang Richard and Anderson, Brian DO and Belhumeur, Peter N},
  year = {2006},
  pages = {1663-1678},
  file = {/Users/e1727/Dropbox/papers/storage/Aspnes et al_2006_A Theory of Network Localization.pdf},
  publisher = {IEEE}
}

@book{Farina2011Positive,
  title = {Positive Linear Systems: Theory and Applications},
  publisher = {{John Wiley \& Sons}},
  author = {Farina, Lorenzo and Rinaldi, Sergio},
  year = {2011}
}

@inproceedings{Azuma2016Structural,
  title = {Structural Bistability Analysis of {{Boolean}} Networks},
  booktitle = {{{IEEE}} 55th {{Conference}} on {{Decision}} and {{Control}}},
  author = {Azuma, Shunichi and Kure, Toshimitsu and Sugie, Toshiharu},
  year = {2016},
  pages = {4833--4836}
}

@article{Arcak2008passivitybased,
  title = {A Passivity-Based Stability Criterion for a Class of Biochemical Reaction Networks},
  volume = {5},
  number = {1},
  journal = {Mathematical biosciences and engineering},
  author = {Arcak, Murat and Sontag, Eduardo},
  year = {2008},
  pages = {1}
}

@book{Frederic2013Modeling,
  title = {Modeling in {{Computational Biology}} and {{Biomedicine}}},
  publisher = {{Springer-Verlag Berlin Heidelberg}},
  author = {Fr{\'e}d{\'e}ric, Cazals and Pierre, Kornprobst},
  year = {2013}
}

@article{Malisoff2006smallgain,
  title = {A Small-Gain Theorem for Motone Systems with Multivalued Input-State Characteristics},
  volume = {51},
  number = {2},
  journal = {IEEE Transactions on Automatic Control},
  author = {Malisoff, Michael and De Leenheer, Patrick},
  year = {2006},
  pages = {287--292}
}

@article{Akian2011Stability,
  title = {Stability and Convergence in Discrete Convex Monotone Dynamical Systems},
  volume = {9},
  issn = {1661-7746},
  abstract = {We study the stable behaviour of discrete dynamical systems where the map is convex and monotone with respect to the standard positive cone. The notion of tangential stability for fixed points and periodic points is introduced, which is weaker than Lyapunov stability. Among others we show that the set of tangentially stable fixed points is isomorphic to a convex inf-semilattice, and a criterion is given for the existence of a unique tangentially stable fixed point. We also show that periods of tangentially stable periodic points are orders of permutations on n letters, where n is the dimension of the underlying space, and a sufficient condition for global convergence to periodic orbits is presented.},
  number = {2},
  journal = {Journal of Fixed Point Theory and Applications},
  doi = {10.1007/s11784-011-0052-1},
  author = {Akian, Marianne and Gaubert, St{\'e}phane and Lemmens, Bas},
  year = {2011},
  pages = {295}
}

@article{Enciso2006Nonmonotone,
  title = {Nonmonotone Systems Decomposable into Monotone Systems with Negative Feedback},
  volume = {224},
  issn = {0022-0396},
  number = {1},
  journal = {Journal of Differential Equations},
  doi = {http://dx.doi.org/10.1016/j.jde.2005.05.007},
  author = {Enciso, G. A. and Smith, H. L. and Sontag, E. D.},
  year = {2006},
  pages = {205 - 227}
}

@article{Sontag1989Smooth,
  title = {Smooth Stabilization Implies Coprime Factorization},
  volume = {34},
  number = {4},
  journal = {IEEE Transactions on Automatic Control},
  author = {Sontag, Eduardo D},
  year = {1989},
  pages = {435--443}
}

@book{OlverNumerical,
  title = {Numerical {{Solution}} of {{Algebraic Systems}}},
  author = {Olver, Peter J}
}

@article{Thron1991secant,
  title = {The Secant Condition for Instability in Biochemical Feedback Control\textemdash{{I}}. {{The}} Role of Cooperativity and Saturability},
  volume = {53},
  number = {3},
  journal = {Bulletin of Mathematical Biology},
  author = {Thron, CD},
  year = {1991},
  pages = {383--401}
}

@article{Mareels1992Monotone,
  title = {Monotone Stability of Nonlinear Feedback Systems},
  volume = {2},
  number = {3},
  journal = {Journal of Mathematical Systems, Estimation, and Control},
  author = {Mareels, Iven MY and Hill, David J},
  year = {1992},
  pages = {275--291}
}

@article{Enciso2006Global,
  title = {Global Attractivity, {{I}}/{{O}} Monotone Small-Gain Theorems, and Biological Delay Systems},
  volume = {14},
  number = {3},
  journal = {Discrete and Continuous Dynamical Systems},
  author = {Enciso, Germ{\'a}n A and Sontag, Eduardo D},
  year = {2006},
  pages = {549}
}

@article{AJiuJinDaYe2008YiChuanZinetutowakunoLiSanmoderutoZhiYu,
  title = {遺伝子ネットワークの離散モデルと制御},
  volume = {47},
  issn = {04534662},
  number = {8},
  journal = {Journal of the Society of Instrument and Control Engineers},
  author = {{阿久津達也}},
  year = {2008},
  pages = {664-669}
}

@book{Poznyak2008Advanced,
  title = {Advanced {{Mathematical Tools}} for {{Automatic Control Engineers}}: {{Deterministic Techniques}}},
  publisher = {{Oxford}},
  author = {Poznyak, Alexander S},
  year = {2008}
}

@article{Morita2013Performance,
  title = {Performance {{Analysis}} of {{Random Dither Quantizers}} in {{Feedback Control Systems}}},
  volume = {6},
  number = {1},
  journal = {SICE Journal of Control, Measurement, and System Integration},
  doi = {10.9746/jcmsi.6.21},
  author = {Morita, Ryosuke and Azuma, Shun-ichi and Sugie, Toshiharu},
  year = {2013},
  pages = {21--27}
}

@article{Piccardi2002Remarks,
  title = {Remarks on Excitability, Stability and Sign of Equilibria in Cooperative Systems},
  volume = {46},
  issn = {0167-6911},
  abstract = {The strict positivity of equilibria is known to be equivalent to asymptotic stability in excitable positive linear systems. In contrast with intuition, this property does not hold for nonlinear cooperative systems. However, weaker results are pointed out and proved to be effective in the analysis of several nonlinear cooperative systems.},
  number = {3},
  journal = {Systems \& Control Letters},
  doi = {http://dx.doi.org/10.1016/S0167-6911(02)00118-4},
  author = {Piccardi, Carlo and Rinaldi, Sergio},
  year = {2002},
  keywords = {Stability,Cooperative systems,Excitability,Positive systems,Positivity of equilibria},
  pages = {153--163}
}

@article{Angeli2014smallgain,
  title = {A Small-Gain Result for Orthant-Monotone Systems under Mixed Feedback},
  volume = {68},
  issn = {0167-6911},
  journal = {Systems \& Control Letters},
  doi = {http://dx.doi.org/10.1016/j.sysconle.2014.03.002},
  author = {Angeli, David and Enciso, Germ{\'a}n A and Sontag, Eduardo D},
  year = {2014},
  keywords = {Global asymptotic stability,Mixed feedback,Monotone systems,Systems biology},
  pages = {9--19}
}

@article{Enciso2005Monotone,
  title = {Monotone Systems under Positive Feedback: Multistability and a Reduction Theorem},
  volume = {54},
  number = {2},
  journal = {Systems \& control letters},
  author = {Enciso, Germ{\'a}n A and Sontag, Eduardo D},
  year = {2005},
  pages = {159--168}
}

@article{Tyson1975existence,
  title = {On the Existence of Oscillatory Solutions in Negative Feedback Cellular Control Processes},
  volume = {1},
  number = {4},
  journal = {Journal of Mathematical Biology},
  author = {Tyson, JJ},
  year = {1975},
  pages = {311--315}
}

@article{Tyson1978dynamics,
  title = {The Dynamics of Feedback Control Circuits in Biochemical Pathways},
  volume = {5},
  number = {1},
  journal = {Progress in Theorretical Biology},
  author = {Tyson, John J and Othmer, Hans G},
  year = {1978},
  pages = {62}
}

@article{JiuLiJunHuang2016YouXianggurahunokakutasuKeKuoDaTiaoJian,
  title = {有向グラフのカクタス可拡大条件},
  journal = {第3回制御部門マルチシンポジウム},
  author = {{久禮俊晃} and {東俊一} and {杉江俊治}},
  year = {2016}
}

@article{Angeli2004smallgain,
  title = {A Small-Gain Theorem for Almost Global Convergence of Monotone Systems},
  volume = {52},
  number = {5},
  journal = {Systems \& control letters},
  author = {Angeli, David and Leenheer, Patrick De and Sontag, Eduardo D},
  year = {2004},
  pages = {407--414}
}

@article{Nishi1984Nonlinear,
  title = {Non-Linear Op-Amp Circuits: {{Existence}} and Uniqueness of Solution by Inspection},
  volume = {12},
  number = {2},
  journal = {International journal of circuit theory and applications},
  author = {Nishi, Tetsuo and Chua, Leon O},
  year = {1984},
  pages = {145--173}
}

@article{Hirsch1988Stability,
  title = {Stability and Convergence in Strongly Monotone Dynamical Systems},
  volume = {383},
  number = {1},
  journal = {Journal f{\"u}r die reine und angewandte Mathematik},
  author = {Hirsch, Morris W},
  year = {1988},
  pages = {53}
}

@article{Paten2011Cactus,
  title = {Cactus Graphs for Genome Comparisons},
  volume = {18},
  number = {3},
  journal = {Journal of Computational Biology},
  author = {Paten, Benedict and Diekhans, Mark and Earl, Dent and John, John St and Ma, Jian and Suh, Bernard and Haussler, David},
  year = {2011},
  pages = {469--481}
}

@article{DeLeenheer2005predatorprey,
  title = {On Predator-Prey Systems and Small-Gain Theorems},
  volume = {2},
  number = {1},
  journal = {Mathematical Biosciences and Engineering},
  author = {De Leenheer, Patrick and Angeli, David and Sontag, Eduardo D},
  year = {2005},
  pages = {25--42}
}

@article{Smith1987Oscillations,
  title = {Oscillations and Multiple Steady States in a Cyclic Gene Model with Repression},
  volume = {25},
  number = {2},
  journal = {Journal of mathematical biology},
  author = {Smith, Hal},
  year = {1987},
  pages = {169--190}
}

@article{Hori2011Existence,
  title = {Existence Criteria of Periodic Oscillations in Cyclic Gene Regulatory Networks},
  volume = {47},
  number = {6},
  journal = {Automatica},
  author = {Hori, Yutaka and Kim, Taehyoung and Hara, Shinji},
  year = {2011},
  pages = {1203--1209}
}

@incollection{Angeli2004Interconnections,
  title = {Interconnections of Monotone Systems with Steady-State Characteristics},
  booktitle = {Optimal Control, Stabilization and Nonsmooth Analysis},
  publisher = {{Springer}},
  author = {Angeli, David and Sontag, Eduardo D},
  year = {2004},
  pages = {135--154}
}

@article{Angeli2004Multistability,
  title = {Multi-Stability in Monotone Input/Output Systems},
  volume = {51},
  number = {3},
  journal = {Systems \& Control Letters},
  author = {Angeli, David and Sontag, Eduardo D},
  year = {2004},
  pages = {185--202}
}

@inproceedings{Ebihara2013Stability,
  title = {Stability and Persistence Analysis of Large Scale Interconnected Positive Systems},
  booktitle = {Control {{Conference}} ({{ECC}}), 2013 {{European}}},
  publisher = {{IEEE}},
  author = {Ebihara, Yoshio and Peaucelle, Dimitri and Arzelier, Denis},
  year = {2013},
  pages = {3366--3371}
}

@article{Arcak2011Diagonal,
  title = {Diagonal Stability on Cactus Graphs and Application to Network Stability Analysis},
  volume = {56},
  number = {12},
  journal = {IEEE Transactions on Automatic Control},
  author = {Arcak, Murat},
  year = {2011},
  pages = {2766--2777}
}

@article{Angeli2008Oscillations,
  title = {Oscillations in {{I}}/{{O}} Monotone Systems under Negative Feedback},
  volume = {53},
  number = {Special Issue},
  journal = {IEEE Transactions on Automatic Control},
  author = {Angeli, David and Sontag, Eduardo D},
  year = {2008},
  pages = {166--176}
}

@article{Mainzer2003Cellular,
  title = {Cellular {{Neural Networks}} and Visual Computing},
  volume = {13},
  number = {01},
  journal = {International Journal of Bifurcation and Chaos},
  author = {Mainzer, Klaus},
  year = {2003},
  pages = {1--6}
}

@book{Jacquez1985Compartmental,
  title = {Compartmental Analysis in Biology and Medicine},
  publisher = {{University of Michigan Press}},
  author = {Jacquez, John A},
  year = {1985}
}

@inproceedings{ElSamad2005Repressilators,
  title = {Repressilators and Promotilators: {{Loop}} Dynamics in Synthetic Gene Networks},
  booktitle = {Proceedings of the 2005, {{American Control Conference}}, 2005.},
  publisher = {{IEEE}},
  author = {El Samad, H and Del Vecchio, D and Khammash, M},
  year = {2005},
  pages = {4405--4410}
}

@article{YiXiong2015JieHeFeiFusisutemunoJieXitoSheJi,
  title = {結合非負システムの解析と設計（特集：非負システムの制御と数理）},
  volume = {59},
  issn = {09161600},
  number = {1},
  journal = {システム/制御/情報 : システム制御情報学会誌},
  author = {義雄, 蛯原},
  year = {1月 2015},
  pages = {21--26}
}

@article{Arcak2006Diagonal,
  title = {Diagonal Stability of a Class of Cyclic Systems and Its Connection with the Secant Criterion},
  volume = {42},
  number = {9},
  journal = {Automatica},
  author = {Arcak, Murat and Sontag, Eduardo D},
  year = {2006},
  pages = {1531--1537}
}

@article{Hirsch2005Monotone,
  title = {Monotone Dynamical Systems},
  volume = {2},
  journal = {Handbook of differential equations: ordinary differential equations},
  author = {Hirsch, Morris W and Smith, Hal},
  year = {2005},
  pages = {239--357}
}

@article{Angeli2003Monotone,
  title = {Monotone Control Systems},
  volume = {48},
  number = {10},
  journal = {IEEE Transactions on Automatic Control},
  author = {Angeli, David and Sontag, Eduardo D},
  year = {2003},
  pages = {1684--1698}
}

@article{Dimarogonas2010Stability,
  title = {Stability Analysis for Multi-Agent Systems Using the Incidence Matrix: Quantized Communication and Formation Control},
  volume = {46},
  number = {4},
  journal = {Automatica},
  author = {Dimarogonas, Dimos V and Johansson, Karl H},
  year = {2010},
  pages = {695--700}
}

@article{Aysal2008Distributed,
  title = {Distributed Average Consensus with Dithered Quantization},
  volume = {56},
  number = {10},
  journal = {IEEE Transactions on Signal Processing},
  author = {Aysal, Tuncer C and Coates, Mark J and Rabbat, Michael G},
  year = {2008},
  pages = {4905--4918}
}

@article{YiDe2013marutiezientosisutemunoZhiYu,
  title = {マルチエージェントシステムの制御 : {{IV}} 合意制御（2）},
  volume = {57},
  issn = {09161600},
  number = {11},
  journal = {システム/制御/情報 : システム制御情報学会誌},
  author = {一徳, 桜間},
  year = {11月 2013},
  pages = {470--479}
}

@article{Lipshitz1992Quantization,
  title = {Quantization and Dither: {{A}} Theoretical Survey},
  volume = {40},
  number = {5},
  journal = {Journal of the Audio Engineering Society},
  author = {Lipshitz, Stanley P and Wannamaker, Robert A and Vanderkooy, John},
  year = {1992},
  pages = {355--375}
}

@book{Godsil2013Algebraic,
  title = {Algebraic Graph Theory},
  volume = {207},
  publisher = {{Springer Science \& Business Media}},
  author = {Godsil, Chris and Royle, Gordon F},
  year = {2013}
}

@article{Widrow2008Quantization,
  title = {Quantization Noise},
  volume = {2},
  journal = {Cambridge University Press},
  author = {Widrow, Bernard and Koll{\'a}r, Istv{\'a}n},
  year = {2008},
  pages = {5}
}

@article{Fiorini1998Motion,
  title = {Motion {{Planning}} in {{Dynamic Environments Using Velocity Obstacles}}},
  volume = {17},
  number = {7},
  journal = {The International Journal of Robotics Research},
  author = {Fiorini, Paolo and Shiller, Zvi},
  year = {1998},
  pages = {760-772},
  publisher = {Sage Publications Sage CA: Thousand Oaks, CA}
}

@article{Bian2010Ising,
  title = {The {{Ising Model}}: {{Teaching}} an {{Old Problem New Tricks}}},
  volume = {2},
  journal = {D-wave systems},
  author = {Bian, Zhengbing and Chudak, Fabian and Macready, William G and Rose, Geordie},
  year = {2010},
  file = {/Users/e1727/Dropbox/papers/storage/The Ising model.pdf}
}

@article{MinZhi2017FeiXianXingmoderuYuCeZhiYunoYanJiuDongXiang,
  title = {非線形モデル予測制御の研究動向},
  volume = {61},
  number = {2},
  journal = {システム／制御／情報},
  doi = {10.11509/isciesci.61.2_42},
  author = {敏之, 大塚},
  year = {2017},
  pages = {42-50},
  file = {/Users/e1727/Dropbox/papers/storage/非線形モデル予測制御の研究動向.pdf}
}

@article{Qin2003survey,
  title = {A {{Survey}} of {{Industrial Model Predictive Control Technology}}},
  volume = {11},
  number = {7},
  journal = {Control Engineering Practice},
  author = {Qin, S Joe and Badgwell, Thomas A},
  year = {2003},
  pages = {733-764},
  file = {/Users/e1727/Dropbox/papers/storage/A survey of industrial model predictive control technology.pdf},
  publisher = {Elsevier}
}

@article{Morari1999Model,
  title = {Model {{Predictive Control}}: {{Past}}, {{Present}} and {{Future}}},
  volume = {23},
  number = {4-5},
  journal = {Computers \& Chemical Engineering},
  author = {Morari, Manfred and Lee, Jay H},
  year = {1999},
  pages = {667-682},
  file = {/Users/e1727/Dropbox/papers/storage/Model predictive control.pdf},
  publisher = {Elsevier}
}

@article{Bemporad1999Control,
  title = {Control of {{Systems Integrating Logic}}, {{Dynamics}}, and {{Constraints}}},
  volume = {35},
  number = {3},
  journal = {Automatica},
  author = {Bemporad, Alberto and Morari, Manfred},
  year = {1999},
  pages = {407-427},
  file = {/Users/e1727/Dropbox/papers/storage/Control of systems integrating logic, dynamics, and constraints.pdf},
  publisher = {Elsevier}
}

@article{Rao1998Application,
  title = {Application of {{Interior}}-{{Point Methods}} to {{Model Predictive Control}}},
  volume = {99},
  number = {3},
  journal = {Journal of optimization theory and applications},
  author = {Rao, Christopher V and Wright, Stephen J and Rawlings, James B},
  year = {1998},
  pages = {723-757},
  file = {/Users/e1727/Dropbox/papers/storage/Application of interior-point methods to model predictive control.pdf},
  publisher = {Springer}
}

@inproceedings{Constantinides2009Tutorial,
  title = {Tutorial {{Paper}}: {{Parallel Architectures}} for {{Model Predictive Control}}},
  booktitle = {Control {{Conference}} ({{ECC}}), 2009 {{European}}},
  author = {Constantinides, George A},
  year = {2009},
  pages = {138-143},
  organization = {IEEE}
}

@book{Desoer1975Feedback,
  title = {Feedback {{Systems}}: {{Input}}-{{Output Properties}}},
  volume = {55},
  publisher = {{Siam}},
  author = {Desoer, Charles A and Vidyasagar, Mathukumalli},
  year = {1975}
}

@article{Nemhauser1988Integer,
  title = {Integer {{Programming}} and {{Combinatorial Optimization}}},
  volume = {20},
  journal = {Wiley, Chichester. GL Nemhauser, MWP Savelsbergh, GS Sigismondi (1992). Constraint Classification for Mixed Integer Programming Formulations. COAL Bulletin},
  author = {Nemhauser, George L and Wolsey, Laurence A},
  year = {1988},
  pages = {8-12},
  file = {/home/e1727/Dropbox/papers/storage/Integer programming and combinatorial optimization.pdf},
  publisher = {Springer}
}

@book{vazirani2013approximation,
  title = {Approximation {{Algorithms}}},
  publisher = {{Springer Science \& Business Media}},
  author = {Vazirani, Vijay V},
  year = {2013}
}

@incollection{Glover1998Tabu,
  title = {Tabu {{Search}}},
  booktitle = {Handbook of Combinatorial Optimization},
  publisher = {{Springer}},
  author = {Glover, Fred and Laguna, Manuel},
  year = {1998},
  pages = {2093-2229},
  file = {/Users/e1727/Dropbox/papers/storage/Tabu Search.pdf}
}

@article{davis1991handbook,
  title = {Handbook of {{Genetic Algorithms}}},
  author = {Davis, Lawrence},
  year = {1991},
  publisher = {CUMINCAD}
}

@article{Suman2006survey,
  title = {A {{Survey}} of {{Simulated Annealing}} as a {{Tool}} for {{Single}} and {{Multiobjective Optimization}}},
  volume = {57},
  number = {10},
  journal = {Journal of the operational research society},
  author = {Suman, Balram and Kumar, Prabhat},
  year = {2006},
  pages = {1143-1160},
  file = {/Users/e1727/Dropbox/papers/storage/A survey of simulated annealing as a tool for single and multiobjective.pdf},
  publisher = {Taylor & Francis}
}

@misc{S.Andersen2004CVXOPT,
  title = {{{CVXOPT}}: {{A Python}} Package for Convex Optimization},
  author = {S. Andersen, Martin and Dahl, Joachim and Vandenberghe, Lieven},
  year = {2004},
  note = {Available at https://cvxopt.org/.}
}

@misc{ohtaman2016anneal,
  title = {Anneal.Py: {{A Python}} Package for Simulated Annealing},
  author = {{ohtaman}},
  year = {2016},
  note = {Available at https://github.com/ohtaman/anneal.}
}

@inproceedings{W.Johnson2018Future,
  address = {{Munich}},
  title = {Future {{Hardware Directions}} of {{Quantum Annealing}}},
  booktitle = {Qubits {{Europe}} 2018 {{D}}-{{Wave Users Conference}}},
  author = {W. Johnson, Mark},
  year = {2018}
}

@patent{Coury2011Graph,
  title = {Graph {{Embedding Techniques}}},
  author = {Coury, Michael and Macready, William G and Grant, David},
  month = jul,
  year = {2011},
  publisher = {Google Patents},
  note = {US Patent 7,984,012}
}

@article{Kadowaki1998Quantum,
  title = {Quantum {{Annealing}} in the {{Transverse Ising Model}}},
  volume = {58},
  number = {5},
  journal = {Physical Review E},
  author = {Kadowaki, Tadashi and Nishimori, Hidetoshi},
  year = {1998},
  pages = {5355},
  file = {/Users/e1727/Dropbox/papers/storage/Quantum annealing in the transverse Ising model.pdf},
  publisher = {APS}
}

@article{Johnson2011Quantum,
  title = {Quantum {{Annealing}} with {{Manufactured Spins}}},
  volume = {473},
  number = {7346},
  journal = {Nature},
  author = {Johnson, Mark W and Amin, Mohammad HS and Gildert, Suzanne and Lanting, Trevor and Hamze, Firas and Dickson, Neil and Harris, R and Berkley, Andrew J and Johansson, Jan and Bunyk, Paul and others},
  year = {2011},
  pages = {194},
  file = {/Users/e1727/Dropbox/papers/storage/Quantum annealing with manufactured spins.pdf},
  publisher = {Nature Publishing Group}
}

@inproceedings{McGeoch2013Experimental,
  title = {Experimental {{Evaluation}} of an {{Adiabiatic Quantum System}} for {{Combinatorial Optimization}}},
  booktitle = {Proceedings of the {{ACM International Conference}} on {{Computing Frontiers}}},
  author = {McGeoch, Catherine C and Wang, Cong},
  year = {2013},
  pages = {23},
  file = {/Users/e1727/Dropbox/papers/storage/McGeoch_Wang_2013_Experimental Evaluation of an Adiabiatic Quantum System for Combinatorial.pdf},
  organization = {ACM}
}

@article{Denchev2016What,
  title = {What {{Is}} the {{Computational Value}} of {{Finite}}-{{Range Tunneling}}?},
  volume = {6},
  number = {3},
  journal = {Physical Review X},
  author = {Denchev, Vasil S and Boixo, Sergio and Isakov, Sergei V and Ding, Nan and Babbush, Ryan and Smelyanskiy, Vadim and Martinis, John and Neven, Hartmut},
  year = {2016},
  pages = {031015},
  publisher = {APS}
}

@article{OMalley2017Nonnegative,
  title = {Nonnegative/Binary Matrix Factorization with a {{D}}-{{Wave}} Quantum Annealer},
  journal = {arXiv preprint arXiv:1704.01605},
  author = {O'Malley, Daniel and Vesselinov, Velimir V and Alexandrov, Boian S and Alexandrov, Ludmil B},
  year = {2017},
  file = {/Users/e1727/Dropbox/papers/storage/Nonnegative-binary matrix factorization with a D-Wave quantum annealer.pdf}
}

@article{Ohzeki2018Optimization,
  title = {Optimization of Neural Networks via Finite-Value Quantum Fluctuations},
  volume = {8},
  number = {1},
  journal = {Scientific reports},
  author = {Ohzeki, Masayuki and Okada, Shuntaro and Terabe, Masayoshi and Taguchi, Shinichiro},
  year = {2018},
  pages = {9950},
  file = {/Users/e1727/Dropbox/papers/storage/Optimization of neural networks via finite-value quantum fluctuations.pdf},
  publisher = {Nature Publishing Group}
}

@inproceedings{Tran2016hybrid,
  title = {A Hybrid Quantum-Classical Approach to Solving Scheduling Problems},
  booktitle = {Ninth {{Annual Symposium}} on {{Combinatorial Search}}},
  author = {Tran, Tony T and Do, Minh and Rieffel, Eleanor G and Frank, Jeremy and Wang, Zhihui and O'Gorman, Bryan and Venturelli, Davide and Beck, J Christopher},
  year = {2016},
  file = {/Users/e1727/Dropbox/papers/storage/A hybrid quantum-classical approach to solving scheduling problems.pdf}
}

@article{Feller1995Constant,
  title = {Constant Pressure Molecular Dynamics Simulation: The {{Langevin}} Piston Method},
  volume = {103},
  number = {11},
  journal = {The Journal of chemical physics},
  author = {Feller, Scott E and Zhang, Yuhong and Pastor, Richard W and Brooks, Bernard R},
  year = {1995},
  pages = {4613-4621},
  file = {/Users/e1727/Dropbox/papers/storage/Constant pressure molecular dynamics simulation.pdf},
  publisher = {AIP}
}

@book{ChaiTianLiangHong2006rubeguJiFenLun,
  title = {ルベーグ積分論},
  isbn = {978-4-7536-0070-0},
  publisher = {{内田老鶴圃}},
  author = {柴田 良弘},
  year = {2006}
}

@article{Le2013Linearquadratic,
  title = {Linear-Quadratic Model Predictive Control for Urban Traffic Networks},
  volume = {80},
  journal = {Procedia-Social and Behavioral Sciences},
  author = {Le, Tung and Vu, Hai L and Nazarathy, Yoni and Vo, Bao and Hoogendoorn, Serge},
  year = {2013},
  pages = {512-530},
  file = {/Users/e1727/Dropbox/papers/storage/Linear-quadratic model predictive control for urban traffic networks.pdf},
  publisher = {Elsevier}
}

@article{Lin2011Fast,
  title = {Fast Model Predictive Control for Urban Road Networks via {{MILP}}},
  volume = {12},
  number = {3},
  journal = {IEEE Transactions on Intelligent Transportation Systems},
  author = {Lin, Shu and De Schutter, Bart and Xi, Yugeng and Hellendoorn, Hans},
  year = {2011},
  pages = {846-856},
  file = {/Users/e1727/Dropbox/papers/storage/Fast model predictive control for urban road networks via MILP.pdf},
  publisher = {IEEE}
}

@article{Camponogara2009Distributed,
  title = {Distributed Optimization for Model Predictive Control of Linear-Dynamic Networks},
  volume = {39},
  number = {6},
  journal = {IEEE Transactions on Systems, Man, and Cybernetics-Part A: Systems and Humans},
  author = {Camponogara, Eduardo and De Oliveira, Lucas Barcelos},
  year = {2009},
  pages = {1331-1338},
  file = {/Users/e1727/Dropbox/papers/storage/Distributed optimization for model predictive control of linear-dynamic networks.pdf},
  publisher = {IEEE}
}

@article{Negenborn2008Multiagent,
  title = {Multi-Agent Model Predictive Control for Transportation Networks: {{Serial}} versus Parallel Schemes},
  volume = {21},
  number = {3},
  journal = {Engineering Applications of Artificial Intelligence},
  author = {Negenborn, Rudy R and De Schutter, Bart and Hellendoorn, J},
  year = {2008},
  pages = {353-366},
  file = {/Users/e1727/Dropbox/papers/storage/Multi-agent model predictive control for transportation networks.pdf},
  publisher = {Elsevier}
}

@article{Aziz2012Unified,
  title = {Unified Framework for Dynamic Traffic Assignment and Signal Control with Cell Transmission Model},
  number = {2311},
  journal = {Transportation Research Record: Journal of the Transportation Research Board},
  author = {Aziz, H and Ukkusuri, Satish},
  year = {2012},
  pages = {73-84},
  file = {/Users/e1727/Dropbox/papers/storage/Aziz_Ukkusuri_2012_Unified framework for dynamic traffic assignment and signal control with cell2.pdf},
  publisher = {Transportation Research Board of the National Academies}
}

@incollection{Tettamanti2010MPC,
  title = {{{MPC}} in Urban Traffic Management},
  booktitle = {Model {{Predictive Control}}},
  publisher = {{InTech}},
  author = {Tettamanti, Tam{\'a}s and Varga, Istv{\'a}n and P{\'e}ni, Tam{\'a}s},
  year = {2010},
  file = {/Users/e1727/Dropbox/papers/storage/MPC in urban traffic management.pdf}
}

@article{Grosso2014Chanceconstrained,
  title = {Chance-Constrained Model Predictive Control for Drinking Water Networks},
  volume = {24},
  number = {5},
  journal = {Journal of process control},
  author = {Grosso, JM and {Ocampo-Mart{\'i}nez}, Carlos and Puig, Vicen{\c c} and Joseph, B},
  year = {2014},
  pages = {504-516},
  publisher = {Elsevier}
}

@inproceedings{Tahersima2010Thermal,
  title = {Thermal Analysis of an Hvac System with Trv Controlled Hydronic Radiator},
  booktitle = {Automation {{Science}} and {{Engineering}} ({{CASE}}), 2010 {{IEEE Conference}} On},
  author = {Tahersima, Fatemeh and Stoustrup, Jakob and Rasmussen, Henrik and Nielsen, Peter Gammeljord},
  year = {2010},
  pages = {756-761},
  file = {/Users/e1727/Dropbox/papers/storage/Thermal analysis of an hvac system with trv controlled hydronic radiator.pdf},
  organization = {IEEE}
}

@inproceedings{Quevedo2003Audio,
  title = {Audio Quantization from a Receding Horizon Control Perspective},
  volume = {5},
  booktitle = {American {{Control Conference}}, 2003. {{Proceedings}} of the 2003},
  author = {Quevedo, Daniel E and Goodwin, Graham C},
  year = {2003},
  pages = {4131-4136},
  file = {/Users/e1727/Dropbox/papers/storage/Audio quantization from a receding horizon control perspective.pdf},
  organization = {IEEE}
}

@inproceedings{Quevedo2002Receding,
  title = {Receding Horizon Linear Quadratic Control with Finite Input Constraint Sets},
  booktitle = {{{IFAC}} 15th {{Triennial World Congress}}},
  author = {Quevedo, Daniel E and De Don{\'a}, Jos{\'e} A and Goodwin, Graham C},
  year = {2002},
  file = {/Users/e1727/Dropbox/papers/storage/Receding horizon linear quadratic control with finite input constraint sets.pdf}
}

@inproceedings{Quevedo2002dynamics,
  title = {On the Dynamics of Receding Horizon Linear Quadratic Finite Alphabet Control Loops},
  volume = {3},
  booktitle = {Decision and {{Control}}, 2002, {{Proceedings}} of the 41st {{IEEE Conference}} On},
  author = {Quevedo, Daniel E and De Dona, Jos{\'e} A and Goodwin, Graham C},
  year = {2002},
  pages = {2929-2934},
  file = {/Users/e1727/Dropbox/papers/storage/On the dynamics of receding horizon linear quadratic finite alphabet control.pdf},
  organization = {IEEE}
}

@book{beantoekusendaru1999QueLuWeiFenFangChengShi,
  address = {{東京}},
  title = {確率微分方程式 : 入門から応用まで},
  isbn = {978-4-431-70804-9},
  publisher = {{シュプリンガー・フェアラーク東京}},
  author = {{ベァーント・エクセンダール}},
  month = mar,
  year = {1999}
}

@article{Wannamaker1992Psychoacoustically,
  title = {Psychoacoustically {{Optimal Noise Shaping}}},
  volume = {40},
  journal = {Journal of the Audio Engineering Society},
  author = {Wannamaker, Rob},
  month = jul,
  year = {1992},
  pages = {611-620},
  file = {/Users/e1727/Dropbox/papers/storage/Psychoacoustically Optimal Noise Shaping.pdf}
}

@book{Pohlmann:2000:PDA:540747,
  edition = {4th},
  title = {Principles of {{Digital Audio}}},
  isbn = {0-07-134819-0},
  publisher = {{McGraw-Hill Professional}},
  author = {Pohlmann, Ken C.},
  year = {2000}
}

@article{Bemporad2002explicit,
  title = {The Explicit Linear Quadratic Regulator for Constrained Systems},
  volume = {38},
  number = {1},
  journal = {Automatica},
  author = {Bemporad, Alberto and Morari, Manfred and Dua, Vivek and Pistikopoulos, Efstratios N},
  year = {2002},
  pages = {3-20},
  file = {/Users/e1727/Dropbox/papers/storage/The explicit linear quadratic regulator for constrained systems.pdf},
  publisher = {Elsevier}
}

@article{XiCun2017noizuniyoruAnDingHua,
  title = {ノイズによる安定化 : 人工ウィーナー過程とその効果に迫る},
  volume = {61},
  issn = {0916-1600},
  number = {9},
  journal = {システム・制御・情報 = Systems, control and information : システム制御情報学会誌},
  author = {西村, 悠樹},
  year = {2017},
  pages = {375-380},
  file = {/Users/e1727/Dropbox/papers/storage/ノイズによる安定化.pdf},
  publisher = {システム制御情報学会}
}

@article{King2015Benchmarking,
  title = {Benchmarking a Quantum Annealing Processor with the Time-to-Target Metric},
  journal = {arXiv preprint arXiv:1508.05087},
  author = {King, James and Yarkoni, Sheir and Nevisi, Mayssam M and Hilton, Jeremy P and McGeoch, Catherine C},
  year = {2015},
  file = {/Users/e1727/Dropbox/papers/storage/Benchmarking a quantum annealing processor with the time-to-target metric.pdf}
}

@article{JingShangDaFu2018LiangZikonpiyutanoYingYongJianTao,
  title = {量子コンピュータの応用検討 -- {{D}}-{{Wave量子アニーラによるモデル予測制御}}},
  journal = {豊田中央研究所研究報告書},
  author = {{井上大輔}},
  year = {2018},
  pages = {201812132}
}

@article{Mitchell2004Introduction,
  title = {Introduction to Digital Audio Coding and Standards},
  volume = {13},
  number = {2},
  journal = {Journal of Electronic Imaging},
  author = {Mitchell, Joan L},
  year = {2004},
  pages = {399},
  publisher = {International Society for Optics and Photonics}
}

@article{Zwicker2013Psychoacoustics,
  title = {Psychoacoustics: {{Facts}} and Models},
  abstract = {Springer Science \& Business Media},
  journal = {Springer Science \& Business Media},
  author = {Zwicker, Eberhard and Fastl, Hugo},
  year = {2013}
}

@article{Mitchell1998Handbook,
  title = {Handbook of {{Genetic Algorithms}}},
  volume = {100},
  journal = {Artif. Intell.},
  author = {Mitchell, Melanie},
  year = {1998},
  pages = {325-330}
}

@article{OGorman2015Bayesian,
  title = {Bayesian Network Structure Learning Using Quantum Annealing},
  volume = {224},
  number = {1},
  journal = {The European Physical Journal Special Topics},
  author = {O'Gorman, Bryan and Babbush, R and {Perdomo-Ortiz}, A and {Aspuru-Guzik}, Al{\'a}n and Smelyanskiy, Vadim},
  year = {2015},
  pages = {163-188},
  file = {/Users/e1727/Dropbox/papers/storage/Bayesian network structure learning using quantum annealing.pdf},
  publisher = {Springer}
}

@article{Venturelli2015Quantum,
  title = {Quantum Annealing Implementation of Job-Shop Scheduling},
  journal = {arXiv preprint arXiv:1506.08479},
  author = {Venturelli, Davide and Marchand, Dominic JJ and Rojo, Galo},
  year = {2015},
  file = {/Users/e1727/Dropbox/papers/storage/Quantum annealing implementation of job-shop scheduling.pdf}
}

@article{Kouro2009Model,
  title = {Model Predictive Control\textemdash{{A}} Simple and Powerful Method to Control Power Converters},
  volume = {56},
  number = {6},
  journal = {IEEE Transactions on industrial electronics},
  author = {Kouro, Samir and Cort{\'e}s, Patricio and Vargas, Ren{\'e} and Ammann, Ulrich and Rodr{\'i}guez, Jos{\'e}},
  year = {2009},
  pages = {1826-1838},
  file = {/Users/e1727/Dropbox/papers/storage/Model predictive control—A simple and powerful method to control power.pdf},
  publisher = {IEEE}
}

@article{Rawlings2000Tutorial,
  title = {Tutorial Overview of Model Predictive Control},
  volume = {20},
  number = {3},
  journal = {IEEE Control Systems},
  author = {Rawlings, James B},
  year = {2000},
  pages = {38-52},
  file = {/Users/e1727/Dropbox/papers/storage/Tutorial overview of model predictive control.pdf},
  publisher = {IEEE}
}

@article{Berg1972Chemotaxis,
  title = {Chemotaxis in {{Escherichia}} Coli Analysed by Three-Dimensional Tracking},
  volume = {239},
  number = {5374},
  journal = {Nature},
  author = {Berg, Howard C and Brown, Douglas A and others},
  year = {1972},
  pages = {500-504},
  file = {/Users/e1727/Dropbox/papers/storage/Chemotaxis in Escherichia coli analysed by three-dimensional tracking.pdf}
}

@misc{Lena,
  title = {Lena},
  howpublished = {https://www.ece.rice.edu/\textasciitilde{}wakin/images/},
  author = {Wakin, Mike},
  year = {2005}
}

@inproceedings{Mondada2009EPuck,
  title = {The {{E}}-{{Puck}}, a {{Robot Designed}} for {{Education}} in {{Engineering}}},
  volume = {1},
  booktitle = {Proceedings of the 9th Conference on Autonomous Robot Systems and Competitions},
  author = {Mondada, Francesco and Bonani, Michael and Raemy, Xavier and Pugh, James and Cianci, Christopher and Klaptocz, Adam and Magnenat, Stephane and Zufferey, Jean-Christophe and Floreano, Dario and Martinoli, Alcherio},
  year = {2009},
  pages = {59-65},
  file = {/Users/e1727/Dropbox/papers/storage/The e-puck, a robot designed for education in engineering.pdf},
  number = {LIS-CONF-2009-004},
  organization = {IPCB: Instituto Politécnico de Castelo Branco}
}

@article{Cortes2004Coverage,
  title = {Coverage {{Control}} for {{Mobile Sensing Networks}}},
  volume = {20},
  number = {2},
  journal = {IEEE Transactions on robotics and Automation},
  author = {Cortes, Jorge and Martinez, Sonia and Karatas, Timur and Bullo, Francesco},
  year = {2004},
  pages = {243-255},
  file = {/Users/e1727/Dropbox/papers/storage/Coverage Control for Mobile Sensing Networks.pdf},
  publisher = {{IEEE}}
}

@article{Martinez2007Motion,
  title = {Motion {{Coordination}} with {{Distributed Information}}},
  volume = {27},
  number = {4},
  journal = {IEEE Control Systems},
  author = {Martinez, Sonia and Cortes, Jorge and Bullo, Francesco},
  year = {2007},
  pages = {75-88},
  file = {/Users/e1727/Dropbox/papers/storage/Motion coordination with distributed information.pdf},
  publisher = {{IEEE}}
}

@article{Olfati-Saber2007Consensus,
  title = {Consensus and {{Cooperation}} in {{Networked Multi}}-{{Agent Systems}}},
  volume = {95},
  number = {1},
  journal = {Proceedings of the IEEE},
  author = {{Olfati-Saber}, Reza and Fax, J Alex and Murray, Richard M},
  year = {2007},
  pages = {215-233},
  file = {/Users/e1727/Dropbox/papers/storage/Consensus and cooperation in networked multi-agent systems.pdf},
  publisher = {{IEEE}}
}

@inproceedings{GaoGangHaoYiLang2006QueLuWeiFenFangChengShi,
  title = {確率微分方程式},
  booktitle = {応用数理サマーセミナー},
  author = {高岡浩一郎},
  year = {2006},
  file = {/Users/e1727/Dropbox/papers/storage/確率微分方程式.pdf}
}

@article{Frangipane2018Dynamic,
  title = {Dynamic Density Shaping of Photokinetic {{E}}. Coli},
  volume = {7},
  journal = {Elife},
  author = {Frangipane, Giacomo and Dell'Arciprete, Dario and Petracchini, Serena and Maggi, Claudio and Saglimbeni, Filippo and Bianchi, Silvio and Vizsnyiczai, Gaszton and Bernardini, Maria Lina and Di Leonardo, Roberto},
  year = {2018},
  pages = {e36608},
  file = {/Users/e1727/Dropbox/papers/storage/Dynamic density shaping of photokinetic E.pdf},
  publisher = {{eLife Sciences Publications Limited}}
}

@article{Slavkov2018Morphogenesisa,
  title = {Morphogenesis in Robot Swarms},
  volume = {3},
  number = {25},
  journal = {Science Robotics},
  author = {Slavkov, I and {Carrillo-Zapata}, D and Carranza, N and Diego, X and Jansson, F and Kaandorp, J and Hauert, S and Sharpe, J},
  year = {2018},
  pages = {eaau9178},
  file = {/Users/e1727/Dropbox/papers/storage/Morphogenesis in robot swarms.pdf},
  publisher = {{Science Robotics}}
}

@article{Alt1980Biased,
  title = {Biased {{Random Walk Models}} for {{Chemotaxis}} and {{Related Diffusion Approximations}}},
  volume = {9},
  issn = {1432-1416},
  abstract = {Stochastic models of biased random walk are discussed, which describe the behavior of chemosensitive cells like bacteria or leukocytes in the gradient of a chemotactic factor. In particular the turning frequency and turn angle distributions are derived from certain biological hypotheses on the background of related experimental observations. Under suitable assumptions it is shown that solutions of the underlying differential-integral equation approximately satisfy the well-known Patlak-Keller-Segel diffusion equation, whose coefficients can be expressed in terms of the microscopic parameters. By an appropriate energy functional a precise error estimation of the diffusion approximation is given within the framework of singular perturbation theory.},
  number = {2},
  journal = {Journal of Mathematical Biology},
  doi = {10.1007/BF00275919},
  author = {Alt, Wolgang},
  month = apr,
  year = {1980},
  pages = {147-177},
  day = {01}
}

@article{Bruna2017Diffusion,
  title = {Diffusion of {{Particles}} with {{Short}}-{{Range Interactions}}},
  volume = {77},
  number = {6},
  journal = {SIAM Journal on Applied Mathematics},
  author = {Bruna, Maria and Chapman, S Jonathan and Robinson, Martin},
  year = {2017},
  pages = {2294-2316},
  file = {/Users/e1727/Dropbox/papers/storage/Diffusion of Particles with Short-Range Interactions.pdf},
  publisher = {{SIAM}}
}

@inproceedings{Cheng2005Robust,
  title = {Robust and Self-Repairing Formation Control for Swarms of Mobile Agents},
  volume = {5},
  booktitle = {{{AAAI}}},
  author = {Cheng, Jimming and Cheng, Winston and Nagpal, Radhika},
  year = {2005},
  file = {/Users/e1727/Dropbox/papers/storage/Robust and self-repairing formation control for swarms of mobile agents.pdf},
  number = {2005}
}

@article{Suzuki2013Chaotic,
  title = {Chaotic {{Ising}}-like Dynamics in Traffic Signals},
  volume = {3},
  journal = {Scientific reports},
  author = {Suzuki, Hideyuki and Imura, Jun-ichi and Aihara, Kazuyuki},
  year = {2013},
  pages = {1127},
  file = {/Users/e1727/Dropbox/papers/storage/Chaotic Ising-like dynamics in traffic signals.pdf},
  publisher = {{Nature Publishing Group}}
}

@article{Robinson2017Particlebased,
  title = {Particle-Based and Meshless Methods with {{Aboria}}},
  volume = {6},
  journal = {SoftwareX},
  author = {Robinson, Martin and Bruna, Maria},
  year = {2017},
  pages = {172-178},
  file = {/Users/e1727/Dropbox/papers/storage/Particle-based and meshless methods with Aboria.pdf},
  publisher = {{Elsevier}}
}

@article{Salazar-Ciudad2003Mechanisms,
  title = {Mechanisms of Pattern Formation in Development and Evolution},
  volume = {130},
  issn = {0950-1991},
  abstract = {We present a classification of developmental mechanisms that have been shown experimentally to generate pattern and form in metazoan organisms. We propose that all such mechanisms can be organized into three basic categories and that two of these may act as composite mechanisms in two different ways. The simple categories are cell autonomous mechanisms in which cells enter into specific arrangements (patterns) without interacting, inductive mechanisms in which cell communication leads to changes in pattern by reciprocal or hierarchical alteration of cell phenotypes (states) and morphogenetic mechanisms in which pattern changes by means of cell interactions that do not change cell states. The latter two types of mechanism can be combined either morphostatically, in which case inductive mechanisms act first, followed by the morphogenetic mechanism, or morphodynamically, in which case both types of mechanisms interact continuously to modify each others dynamics. We propose that this previously unexplored distinction in the operation of composite developmental mechanisms provides insight into the dynamics of many developmental processes. In particular, morphostatic and morphodynamic mechanisms respond to small changes in their genetic and microenvironmental components in dramatically different ways. We suggest that these differences in variational properties lead to morphostatic and morphodynamic mechanisms being represented to different extents in early and late stages of development and to their contributing in distinct ways to morphological transitions in evolution.},
  number = {10},
  journal = {Development},
  doi = {10.1242/dev.00425},
  author = {{Salazar-Ciudad}, Isaac and Jernvall, Jukka and Newman, Stuart A.},
  year = {2003},
  pages = {2027-2037},
  file = {/Users/e1727/Dropbox/papers/storage/Mechanisms of pattern formation in development and evolution.pdf},
  publisher = {{The Company of Biologists Ltd}},
  eprint = {http://dev.biologists.org/content/130/10/2027.full.pdf}
}

@article{DinoueDistributed22018,
  title = {群ロボットシステムの分散自己位置推定 第 2 報　数値計算と実機実験による性能評価},
  journal = {豊田中央研究所研究報告書},
  author = {井上大輔},
  year = {2018},
  pages = {201807127}
}

@inproceedings{Izumi2014Coverage,
  title = {Coverage {{Control Inspired}} by {{Bacterial Chemotaxis}}},
  abstract = {This paper considers distributed control of multi-agent systems, inspired by chemotaxis of bacteria. The chemotaxis is the biological phenomenon that organisms sense the concentration of a chemical in an environment and move toward or away from the highest concentration point. The problem considered here is a coverage problem, i.e., a problem of finding distributed controllers to steer agents so that they are placed uniformly on a given space. As a solution to this problem, we propose distributed controllers based on the mechanism of the chemotaxis. With the proposed controllers, each agent performs forward movement or random rotation depending on the difference between the current achievement degree of the coverage and the previous one. The performance of the proposed controllers is demonstrated by a numerical experiment. This result shows that multi-agent coordination in a distributed manner can be achieved by using the mechanism of the chemotaxis.},
  booktitle = {2014 {{IEEE}} 33rd {{International Symposium}} on {{Reliable Distributed Systems Workshops}}},
  doi = {10.1109/SRDSW.2014.11},
  author = {Izumi, S. and Azuma, S. and Sugie, T.},
  month = oct,
  year = {2014},
  keywords = {distributed control,bacterial chemotaxis,biological phenomenon,biology,cell motility,Chemicals,chemotaxis,Control systems,coverage control,microorganisms,Microorganisms,multi-agent systems,Multi-agent systems,multiagent coordination,multiagent system distributed control,Performance analysis,Robots},
  pages = {34-39},
  file = {/Users/e1727/Dropbox/papers/storage/Coverage Control Inspired by Bacterial Chemotaxis.pdf;/Users/e1727/Dropbox/Zotero/storage/FLMWSHED/7000133.html}
}

@article{Yang2015Selforganized,
  title = {Self-Organized Swarm Robot for Target Search and Trapping Inspired by Bacterial Chemotaxis},
  volume = {72},
  issn = {0921-8890},
  abstract = {Target search and trapping using self-organized swarm robots have received increasing attention in recent years but control design of these systems remains a challenge. In this paper, we propose a decentralized control algorithm of swarm robot for target search and trapping inspired by bacteria chemotaxis. First, a local coordinate system is established according to the initial positions of the robots in the target area. Then the target area is divided into Voronoi cells. After the initialization, swarm robots start performing target search and trapping missions driven by the proposed bacteria chemotaxis algorithm under the guidance of the gradient information defined by the target. Simulation results demonstrate the effectiveness of the algorithm and its robustness to unexpected robot failure. Compared with other commonly used methods for distributed control of swarm robots, our simulation results indicate that the bacteria chemotaxis algorithm exhibits less vulnerability to local optimum, and high computational efficiency.},
  journal = {Robotics and Autonomous Systems},
  doi = {10.1016/j.robot.2015.05.001},
  author = {Yang, Bin and Ding, Yongsheng and Jin, Yaochu and Hao, Kuangrong},
  month = oct,
  year = {2015},
  keywords = {Distributed control,Bacteria chemotaxis,Self-organization,Swarm robots,Target searching,Target trapping},
  pages = {83-92},
  file = {/Users/e1727/Dropbox/papers/storage/Self-organized swarm robot for target search and trapping inspired by bacterial.pdf;/Users/e1727/Dropbox/Zotero/storage/HXXXM5U3/S0921889015000937.html}
}

@article{Meng2013morphogenetic,
  title = {A Morphogenetic Approach to Flexible and Robust Shape Formation for Swarm Robotic Systems},
  volume = {61},
  issn = {0921-8890},
  abstract = {Embryonic development of multi-cellular organisms is governed by gene regulatory networks (GRNs), which are a collection of genes that interact with one another and with other chemicals in the cell. Inspired by the morphogenesis of biological organisms, in this paper, we propose a morphogenetic approach using a gene regulatory network (GRN) for swarm robotic systems to form complex shapes in a distributed manner. The target pattern, represented by non-uniform rational B-spline (NURBS), is embedded into the gene regulatory model, analogous to the morphogen gradients in multi-cellular development. Since the total number of robots is unknown to each robot, a dynamic neighborhood adaptation mechanism is proposed to evenly deploy the robots on the boundary of the target pattern. A theoretical proof of the system convergence is provided. Various simulation studies demonstrate that the proposed algorithm offers an effective and robust distributed control mechanism for swarm robotic systems to construct complex shapes. Furthermore, proof-of-concept experiments were successfully undertaken using e-puck mobile robots, which demonstrate that the proposed model works well with physical constraints of real robots.},
  number = {1},
  journal = {Robotics and Autonomous Systems},
  doi = {10.1016/j.robot.2012.09.009},
  author = {Meng, Yan and Guo, Hongliang and Jin, Yaochu},
  month = jan,
  year = {2013},
  keywords = {Self-organization,Swarm robots,Distributed systems,Gene regulatory network,Morphogenesis,Shape formation},
  pages = {25-38},
  file = {/Users/e1727/Dropbox/papers/storage/A morphogenetic approach to flexible and robust shape formation for swarm.pdf;/Users/e1727/Dropbox/papers/storage/A morphogenetic approach to flexible and robust shape formation for swarm.pdf;/Users/e1727/Dropbox/Zotero/storage/6CG2XSFU/S0921889012001637.html}
}

@article{Liu2019Swarm,
  title = {Swarm Intelligence Inspired Cooperation Promotion and Symmetry Breaking in Interdependent Networked Game},
  volume = {29},
  issn = {1054-1500},
  abstract = {The evolution of a cooperative strategy on multilayer networks is arousing increasing concern. Most of the previous studies assumed that agents can only choose cooperation or defection when interacting with their partners, whereas the actual provisions in real world scenarios might not be discrete, but rather continuous. Furthermore, in evolutionary game, agents often make use of their memory which keeps the most successful strategy in the past, as well as the best current strategy gained by their directed neighbors, to find the best available strategies. Inspired by these observations, we study the impact of the particle swarm optimization (PSO) algorithm on the evolution of cooperation on interdependent networks in the continuous version of spatial prisoner's dilemma games. Following extensive simulations of this setup, we can observe that the introduction of the PSO mechanism on the interdependent networks can promote cooperation strongly, regardless of the network coupling strength. In addition, we find that the increment of coupling strength is more suitable for the propagation of cooperation. More interestingly, we find that when the coupling strength is relatively large, a spontaneous symmetry breaking phenomenon of cooperation occurs between the interdependent networks. To interpret the symmetry breaking phenomenon, we investigate the asynchronous expansion of heterogeneous strategy couples between different networks. Since this work takes cooperation from a more elaborate perspective, we believe that it may provide a deep understanding of the evolution of cooperation in social networks.},
  number = {4},
  journal = {Chaos: An Interdisciplinary Journal of Nonlinear Science},
  doi = {10.1063/1.5088932},
  author = {Liu, Yishun and Yang, Chunhua and Huang, Keke and Wang, Zhen},
  month = apr,
  year = {2019},
  pages = {043101},
  file = {/Users/e1727/Dropbox/papers/storage/Swarm intelligence inspired cooperation promotion and symmetry breaking in.pdf;/Users/e1727/Dropbox/Zotero/storage/N3X5K8GB/1.html}
}

@article{Hussein2007Effective,
  title = {Effective {{Coverage Control}} for {{Mobile Sensor Networks With Guaranteed Collision Avoidance}}},
  volume = {15},
  issn = {1063-6536},
  abstract = {This paper studies the problem of dynamically covering a given region in the plane using a set of mobile sensor agents. A novel problem formulation is proposed that addresses a number of important multiagent missions. The coverage goal, which is to cover a given search domain using multiple mobile sensors such that each point is surveyed until a certain preset level is achieved, is formulated in a mathematically precise problem statement. A control law is developed that guarantees to meet the coverage goal. This control law is modified to guarantee that a partially connected fleet also attains the coverage goal. Finally, a collision avoidance component is added to the controller to guarantee that the agents do not collide. The new controller is shown to safely achieve coverage. Several numerical examples are provided to illustrate the main results.},
  number = {4},
  journal = {IEEE Transactions on Control Systems Technology},
  doi = {10.1109/TCST.2007.899155},
  author = {Hussein, I. I. and Stipanovic, D. M.},
  month = jul,
  year = {2007},
  keywords = {telecommunication control,wireless sensor networks,Collision avoidance,mobile communication,Wireless sensor networks,sensors,sensor networks,Mobile communication,collision avoidance,Humans,Communication system control,Cooperative systems,Control systems,coverage control,multi-agent systems,cooperative system,cooperative systems,mobile sensor agent,mobile sensor network,mobile sensor systems,multiagent missions,multisensor systems,Multisensor systems,Sensor systems,Space missions},
  pages = {642-657},
  file = {/Users/e1727/Dropbox/Zotero/storage/J2XYUG6U/4252099.html}
}

@article{Choset2001Coverage,
  title = {Coverage for Robotics \textendash{} {{A}} Survey of Recent Results},
  volume = {31},
  issn = {1573-7470},
  abstract = {This paper surveys recent results in coverage path planning, a new path planning approach that determines a path for a robot to pass over all points in its free space. Unlike conventional point-to-point path planning, coverage path planning enables applications such as robotic de-mining, snow removal, lawn mowing, car-body painting, machine milling, etc. This paper will focus on coverage path planning algorithms for mobile robots constrained to operate in the plane. These algorithms can be classified as either heuristic or complete. It is our conjecture that most complete algorithms use an exact cellular decomposition, either explicitly or implicitly, to achieve coverage. Therefore, this paper organizes the coverage algorithms into four categories: heuristic, approximate, partial-approximate and exact cellular decompositions. The final section describes some provably complete multi-robot coverage algorithms.},
  language = {en},
  number = {1},
  journal = {Annals of Mathematics and Artificial Intelligence},
  doi = {10.1023/A:1016639210559},
  author = {Choset, Howie},
  month = oct,
  year = {2001},
  keywords = {mobile robots,cell decompositions,coverage},
  pages = {113-126}
}

@inproceedings{InoueDistributed2019,
  address = {{Prague}},
  title = {Distributed {{Range}}-Based {{Localization}} for {{Swarm Robot Systems}} Using {{Sensor}}-{{Fusion}} Technique},
  booktitle = {{{SENSORNETS2019}}},
  author = {Inoue, Daisuke and Murai, Daisuke and Ikuta, Yasuhiro and Horoaki, Yoshida},
  year = {2019}
}

@article{DAPONTE20133291,
  title = {State of the Art and Future Developments of Measurement Applications on Smartphones},
  volume = {46},
  issn = {0263-2241},
  abstract = {The modern smartphones contain different sensor technologies, so they can be used as stand-alone measurement instruments on a wide range of application domains. The paper deals with a survey of measurement applications based on smartphones. In the first part, the evolution of mobile phone technologies, including the sensors and mobile networks developments, is presented. Then, in order to highlight the sensors and the communication capabilities, the architectural overview of the hardware and software technologies, which are available on latest series of smartphones, is reported and discussed. A review of measurements applications using the smart sensors and the communication interfaces available on smartphones, it is also presented. A classification of smartphone applications, which looks the smartphone as a handheld measurement instrument, is presented. In the last part, the integration of augmented reality to the measurement applications and new type of measurement systems, having a smartphone as processing support, is presented.},
  number = {9},
  journal = {Measurement},
  doi = {https://doi.org/10.1016/j.measurement.2013.05.006},
  author = {Daponte, P. and Vito, L. De and Picariello, F. and Riccio, M.},
  year = {2013},
  keywords = {Augmented reality,Measurement application,Smart sensor,Smartphone},
  pages = {3291-3307}
}

@article{Guo2012Morphogenetic,
  title = {A {{Morphogenetic Framework}} for {{Self}}-Organized {{Multirobot Pattern Formation}} and {{Boundary Coverage}}},
  volume = {7},
  issn = {1556-4665},
  abstract = {Embryonic development of multicellular organisms, also known as morphogenesis, is regarded as a robust self-organization process for pattern generation. Inspired by the recent findings in biology indicating that morphogen gradients, together with a Gene Regulatory Network (GRN), play a key role in biological patterning, we propose a framework for self-organized multirobot pattern formation and boundary coverage based on an artificial GRN model. The proposed framework does not need a global coordinate system, which makes it more practical to be implemented in a physical robotic system. Moreover, an adaptation mechanism is included in the framework so that the self-organization algorithm is robust to changes in the number of robots. Various case studies of multirobot pattern formation and boundary coverage show the effectiveness of the framework.},
  number = {1},
  journal = {ACM Trans. Auton. Adapt. Syst.},
  doi = {10.1145/2168260.2168275},
  author = {Guo, Hongliang and Jin, Yaochu and Meng, Yan},
  month = may,
  year = {2012},
  keywords = {boundary coverage,morphogenesis,self-organization,shape formation,Swarm robotic systems},
  pages = {15:1--15:23},
  file = {/Users/e1727/Dropbox/papers/storage/A Morphogenetic Framework for Self-organized Multirobot Pattern Formation and.pdf}
}

@misc{Ising,
  title = {An {{Ising Model}} for {{Road Traffic Inference}} | {{Paper}} | {{Microsoft Academic}}},
  howpublished = {https://academic.microsoft.com/paper/1606246638/reference/search?q=An\%20Ising\%20Model\%20for\%20Road\%20Traffic\%20Inference\&qe=Or(Id\%253D2137813581\%252CId\%253D2165232124\%252CId\%253D2128084896\%252CId\%253D1971565000\%252CId\%253D2112036188\%252CId\%253D118011060\%252CId\%253D2098678088\%252CId\%253D1934021597\%252CId\%253D2158122241\%252CId\%253D1523363508\%252CId\%253D2118696796\%252CId\%253D2167567449\%252CId\%253D67367170\%252CId\%253D2043014754\%252CId\%253D1977327092\%252CId\%253D2109091716\%252CId\%253D2153053671\%252CId\%253D1604803556\%252CId\%253D2112689294\%252CId\%253D1985813166\%252CId\%253D1484743436\%252CId\%253D2099164281\%252CId\%253D2115425194\%252CId\%253D2170420203\%252CId\%253D1986202807\%252CId\%253D1981392829\%252CId\%253D2054966400\%252CId\%253D2058252247\%252CId\%253D2021324855\%252CId\%253D2014662635\%252CId\%253D2069097920)\&f=\&orderBy=0},
  file = {/Users/e1727/Dropbox/Zotero/storage/MLSTM6EA/search.html}
}

@article{nagatani2009freezing,
  title = {Freezing Transition in the Mean-Field Approximation Model of Pedestrian Counter Flow},
  volume = {388},
  number = {24},
  journal = {Physica A: Statistical Mechanics and its Applications},
  author = {Nagatani, Takashi},
  year = {2009},
  pages = {4973-4978},
  file = {/Users/e1727/Dropbox/papers/storage/Freezing transition in the mean-field approximation model of pedestrian counter.pdf},
  publisher = {{Elsevier}}
}

@article{Muramatsu1999Jamming,
  title = {Jamming Transition in Pedestrian Counter Flow},
  volume = {267},
  issn = {0378-4371},
  abstract = {A lattice gas model with biased random walkers is presented to mimic the pedestrian counter flow in a channel under the open boundary condition of constant density. There are two types of walkers without the back step: the one is the random walker going to the right and the other is the random walker going to the left. It is found that a dynamical jamming transition from the freely moving state at low density to the stopped state at high density occurs at the critical density. The transition point is given by pc=0.45{$\pm$}0.01, not depending on the system size. The transition point depends on the strength of drift and decreases with increasing drift. Also, we present the extended model to take into account the traffic rule in which a pedestrian walks preferably on the right-hand side of the channel.},
  number = {3},
  journal = {Physica A: Statistical Mechanics and its Applications},
  doi = {10.1016/S0378-4371(99)00018-7},
  author = {Muramatsu, Masakuni and Irie, Tunemasa and Nagatani, Takashi},
  month = may,
  year = {1999},
  keywords = {Pedestrian flow,Phase transition,Traffic flow},
  pages = {487-498},
  file = {/Users/e1727/Dropbox/papers/storage/Jamming transition in pedestrian counter flow.pdf;/Users/e1727/Dropbox/Zotero/storage/U4UUV2GZ/S0378437199000187.html}
}

@inproceedings{chevalier2015micro,
  title = {A Micro-Macro Traffic Model Based on Mean-Field Games},
  booktitle = {2015 {{American Control Conference}} ({{ACC}})},
  author = {Chevalier, Geoffroy and Le Ny, Jerome and Malham{\'e}, Roland},
  year = {2015},
  pages = {1983-1988},
  file = {/Users/e1727/Dropbox/papers/storage/A micro-macro traffic model based on mean-field games.pdf},
  organization = {{IEEE}}
}

@article{Schadschneider2002Traffic,
  series = {Fundamental {{Problems}} in {{Statistical Physics}}},
  title = {Traffic Flow: A Statistical Physics Point of View},
  volume = {313},
  issn = {0378-4371},
  shorttitle = {Traffic Flow},
  abstract = {The investigation of traffic flow problems has a long tradition and various methods and approaches have been applied. In this review we focus on statistical mechanics and nonequilibrium aspects. It is shown that many properties of traffic flow can be modelled successfully by using rather simple cellular automaton models. Analytical methods for the investigation of discrete models are presented in some detail. Apart from highway traffic, also the modelling of city traffic and pedestrian dynamics will be discussed.},
  number = {1},
  journal = {Physica A: Statistical Mechanics and its Applications},
  doi = {10.1016/S0378-4371(02)01036-1},
  author = {Schadschneider, Andreas},
  month = oct,
  year = {2002},
  keywords = {Cellular automata,Complex systems,Nonequilibrium physics},
  pages = {153-187},
  file = {/Users/e1727/Dropbox/papers/storage/Traffic flow.pdf;/Users/e1727/Dropbox/Zotero/storage/XRH26F6W/S0378437102010361.html}
}

@article{bensoussan2016linear,
  title = {Linear-Quadratic Mean Field Games},
  volume = {169},
  number = {2},
  journal = {Journal of Optimization Theory and Applications},
  author = {Bensoussan, Alain and Sung, KCJ and Yam, Sheung Chi Phillip and Yung, Siu-Pang},
  year = {2016},
  pages = {496-529},
  file = {/Users/e1727/Dropbox/papers/storage/Linear-quadratic mean field games.pdf},
  publisher = {{Springer}}
}

@book{bensoussan2013mean,
  title = {Mean Field Games and Mean Field Type Control Theory},
  volume = {101},
  publisher = {{Springer}},
  author = {Bensoussan, Alain and Frehse, Jens and Yam, Phillip and others},
  year = {2013},
  file = {/Users/e1727/Dropbox/papers/storage/Mean field games and mean field type control theory.pdf}
}

@article{Huang2019GameTheoretic,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1903.06053},
  primaryClass = {physics},
  title = {A {{Game}}-{{Theoretic Framework}} for {{Autonomous Vehicles Velocity Control}}: {{Bridging Microscopic Differential Games}} and {{Macroscopic Mean Field Games}}},
  shorttitle = {A {{Game}}-{{Theoretic Framework}} for {{Autonomous Vehicles Velocity Control}}},
  abstract = {A transportation system with fully autonomous vehicles can be modeled as a multi-agent system, where autonomous vehicles interact with one another through coupled optimal driving strategies. However, the existing literature on autonomous vehicle longitudinal control suffers from scalability issues. In other words, it is challenging to deploy these control algorithms to a large number of autonomous vehicles. This paper aims to tackle such a challenge by employing mean field approximation and deriving a macroscopic game-theoretic framework for autonomous vehicles traffic flow from microscopic velocity control. The developed game is "mean field game (MFG)", which is essentially the limiting differential game with an infinite number of agents. It is a micro-macro model which allows one to define individuals on a microscopic level as rational utility-optimizing agents while translating rich microscopic behaviors to macroscopic models. Despite a few studies on the application of MFG to traffic flow models, this paper offers a systematic framework to apply MFG to autonomous vehicle control from four aspects: (i) We first derive the mean field game as a continuum version of discrete differential game; (ii) We develop a solution algorithm based on multigrid preconditioned Newton's method to solve a mean field equilibrium; (iii) We construct a tuple of discrete controls from the continuous mean field equilibrium and demonstrates its accuracy as an \$\textbackslash{}epsilon\$-Nash equilibrium to the original discrete differential game, so that those controls can be deployed to individual autonomous vehicles in the context of discrete games. (iv) The derived mean field game can also be treated as a macroscopic traffic flow model. We show its connections to traditional LWR model and present some examples to illustrate traffic flow characteristics of mean field game.},
  journal = {arXiv:1903.06053 [physics]},
  author = {Huang, Kuang and Di, Xuan and Du, Qiang and Chen, Xi},
  month = mar,
  year = {2019},
  keywords = {Computer Science - Systems and Control,Mathematics - Optimization and Control,Physics - Physics and Society},
  file = {/Users/e1727/Dropbox/papers/storage/Huang et al_2019_A Game-Theoretic Framework for Autonomous Vehicles Velocity Control.pdf;/Users/e1727/Dropbox/Zotero/storage/UTHU3FL3/Huang et al. - 2019 - A Game-Theoretic Framework for Autonomous Vehicles.pdf;/Users/e1727/Dropbox/Zotero/storage/K8QMIYAA/1903.html}
}

@article{daganzo2006traffic,
  title = {In Traffic Flow, Cellular Automata= Kinematic Waves},
  volume = {40},
  number = {5},
  journal = {Transportation Research Part B: Methodological},
  author = {Daganzo, Carlos F},
  year = {2006},
  pages = {396-403},
  file = {/Users/e1727/Dropbox/papers/storage/In traffic flow, cellular automata= kinematic waves.pdf;/Users/e1727/Dropbox/papers/storage/In traffic flow, cellular automata= kinematic waves2.pdf},
  publisher = {{Elsevier}}
}

@article{LighthillMichaelJames1955kinematic,
  title = {On Kinematic Waves {{II}}. {{A}} Theory of Traffic Flow on Long Crowded Roads},
  volume = {229},
  abstract = {This paper uses the method of kinematic waves, developed in part I, but may be read independently. A functional relationship between flow and concentration for traffic on crowded arterial roads has been postulated for some time, and has experimental backing (\textsection{}2). From this a theory of the propagation of changes in traffic distribution along these roads may be deduced (\textsection\textsection{}2, 3). The theory is applied (\textsection{}4) to the problem of estimating how a `hump', or region of increased concentration, will move along a crowded main road. It is suggested that it will move slightly slower than the mean vehicle speed, and that vehicles passing through it will have to reduce speed rather suddenly (at a `shock wave') on entering it, but can increase speed again only very gradually as they leave it. The hump gradually spreads out along the road, and the time scale of this process is estimated. The behaviour of such a hump on entering a bottleneck, which is too narrow to admit the increased flow, is studied (\textsection{}5), and methods are obtained for estimating the extent and duration of the resulting hold-up. The theory is applicable principally to traffic behaviour over a long stretch of road, but the paper concludes (\textsection{}6) with a discussion of its relevance to problems of flow near junctions, including a discussion of the starting flow at a controlled junction. In the introductory sections 1 and 2, we have included some elementary material on the quantitative study of traffic flow for the benefit of scientific readers unfamiliar with the subject.},
  number = {1178},
  journal = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
  doi = {10.1098/rspa.1955.0089},
  author = {{Lighthill Michael James} and {Whitham Gerald Beresford}},
  month = may,
  year = {1955},
  pages = {317-345},
  file = {/Users/e1727/Dropbox/papers/storage/On kinematic waves II.pdf;/Users/e1727/Dropbox/Zotero/storage/DVVYY6A6/rspa.1955.html}
}

@article{KachrooInverse2016,
  title = {Inverse {{Problem}} for {{Non}}-{{Viscous Mean Field Control}}: {{Example From Traffic}}},
  volume = {61},
  issn = {0018-9286},
  shorttitle = {Inverse {{Problem}} for {{Non}}-{{Viscous Mean Field Control}}},
  abstract = {This paper presents an inverse problem for mean field games where we find the mean field problem statement for which the given dynamics is the solution. We use distributed traffic as an example and derive the classic Lighthill Whitham Richards (LWR) model as a solution of the non-viscous mean field game. We also derive the same model by choosing a different problem where we use travel time, which is a distributed parameter, as the cost for the optimal control. We then study the stationary versions of these two problems and provide numerical solutions for the same.},
  number = {11},
  journal = {IEEE Transactions on Automatic Control},
  doi = {10.1109/TAC.2015.2511929},
  author = {Kachroo, P. and Agarwal, S. and Sastry, S.},
  month = nov,
  year = {2016},
  keywords = {Vehicles,optimal control,Mathematical model,distributed parameter,distributed traffic,FPK,game theory,Games,HJB,inverse problem,inverse problems,Inverse problems,Lighthill Whitham Richards,LWR,LWR model,mean field games,mean field problem statement,Microscopy,nonviscous mean field control,nonviscous mean field game,Numerical models,numerical solutions,traffic control,traffic modeling,travel time,Vehicle dynamics},
  pages = {3412-3421},
  file = {/Users/e1727/Dropbox/papers/storage/Inverse Problem for Non-Viscous Mean Field Control.pdf;/Users/e1727/Dropbox/papers/storage/Inverse Problem for Non-Viscous Mean Field Control2.pdf;/Users/e1727/Dropbox/Zotero/storage/Q6YNTVFT/7364206.html;/Users/e1727/Dropbox/Zotero/storage/UGITCWYW/7364206.html}
}

@article{Mguni2018Decentralised,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1803.05028},
  primaryClass = {cs},
  title = {Decentralised {{Learning}} in {{Systems}} with {{Many}}, {{Many Strategic Agents}}},
  abstract = {Although multi-agent reinforcement learning can tackle systems of strategically interacting entities, it currently fails in scalability and lacks rigorous convergence guarantees. Crucially, learning in multi-agent systems can become intractable due to the explosion in the size of the state-action space as the number of agents increases. In this paper, we propose a method for computing closed-loop optimal policies in multi-agent systems that scales independently of the number of agents. This allows us to show, for the first time, successful convergence to optimal behaviour in systems with an unbounded number of interacting adaptive learners. Studying the asymptotic regime of N-player stochastic games, we devise a learning protocol that is guaranteed to converge to equilibrium policies even when the number of agents is extremely large. Our method is model-free and completely decentralised so that each agent need only observe its local state information and its realised rewards. We validate these theoretical results by showing convergence to Nash-equilibrium policies in applications from economics and control theory with thousands of strategically interacting agents.},
  journal = {arXiv:1803.05028 [cs]},
  author = {Mguni, David and Jennings, Joel and {de Cote}, Enrique Munoz},
  month = mar,
  year = {2018},
  keywords = {Computer Science - Multiagent Systems},
  file = {/Users/e1727/Dropbox/papers/storage/Inverse Problem for Non-Viscous Mean Field Control.pdf;/Users/e1727/Dropbox/Zotero/storage/LDMUHDHM/Mguni et al. - 2018 - Decentralised Learning in Systems with Many, Many .pdf;/Users/e1727/Dropbox/Zotero/storage/2U3WXRA4/1803.html}
}

@article{Ito2015Maxwell,
  title = {Maxwell's Demon in Biochemical Signal Transduction with Feedback Loop},
  volume = {6},
  copyright = {2015 Nature Publishing Group},
  issn = {2041-1723},
  abstract = {Signal transduction in living cells is vital to maintain life itself, where information transfer in noisy environment plays a significant role. In a rather different context, the recent intensive research on `Maxwell's demon'\textemdash{}a feedback controller that utilizes information of individual molecules\textemdash{}have led to a unified theory of information and thermodynamics. Here we combine these two streams of research, and show that the second law of thermodynamics with information reveals the fundamental limit of the robustness of signal transduction against environmental fluctuations. Especially, we find that the degree of robustness is quantitatively characterized by an informational quantity called transfer entropy. Our information-thermodynamic approach is applicable to biological communication inside cells, in which there is no explicit channel coding in contrast to artificial communication. Our result could open up a novel biophysical approach to understand information processing in living systems on the basis of the fundamental information\textendash{}thermodynamics link.},
  language = {en},
  journal = {Nature Communications},
  doi = {10.1038/ncomms8498},
  author = {Ito, Sosuke and Sagawa, Takahiro},
  month = jun,
  year = {2015},
  pages = {7498},
  file = {/Users/e1727/Dropbox/papers/storage/Maxwell’s demon in biochemical signal transduction with feedback loop.pdf;/Users/e1727/Dropbox/papers/storage/Maxwell’s demon in biochemical signal transduction with feedback loop2.pdf;/Users/e1727/Dropbox/Zotero/storage/DT3LCJ6M/ncomms8498.html}
}

@article{Bergdorf2010Lagrangian,
  title = {A {{Lagrangian}} Particle Method for Reaction\textendash{}Diffusion Systems on Deforming Surfaces},
  volume = {61},
  issn = {1432-1416},
  abstract = {Reaction\textendash{}diffusion processes on complex deforming surfaces are fundamental to a number of biological processes ranging from embryonic development to cancer tumor growth and angiogenesis. The simulation of these processes using continuum reaction\textendash{}diffusion models requires computational methods capable of accurately tracking the geometric deformations and discretizing on them the governing equations. We employ a Lagrangian level-set formulation to capture the deformation of the geometry and use an embedding formulation and an adaptive particle method to discretize both the level-set equations and the corresponding reaction\textendash{}diffusion. We validate the proposed method and discuss its advantages and drawbacks through simulations of reaction\textendash{}diffusion equations on complex and deforming geometries.},
  language = {en},
  number = {5},
  journal = {Journal of Mathematical Biology},
  doi = {10.1007/s00285-009-0315-2},
  author = {Bergdorf, Michael and Sbalzarini, Ivo F. and Koumoutsakos, Petros},
  month = nov,
  year = {2010},
  keywords = {35Q92,76M28,92C15},
  pages = {649-663},
  file = {/Users/e1727/Dropbox/papers/storage/Bergdorf et al_2010_A Lagrangian particle method for reaction–diffusion systems on deforming.pdf;/Users/e1727/Dropbox/papers/storage/Bergdorf et al_2010_A Lagrangian particle method for reaction–diffusion systems on deforming2.pdf}
}

@article{Barbosa2018Human,
  series = {Human Mobility: {{Models}} and Applications},
  title = {Human Mobility: {{Models}} and Applications},
  volume = {734},
  issn = {0370-1573},
  shorttitle = {Human Mobility},
  abstract = {Recent years have witnessed an explosion of extensive geolocated datasets related to human movement, enabling scientists to quantitatively study individual and collective mobility patterns, and to generate models that can capture and reproduce the spatiotemporal structures and regularities in human trajectories. The study of human mobility is especially important for applications such as estimating migratory flows, traffic forecasting, urban planning, and epidemic modeling. In this survey, we review the approaches developed to reproduce various mobility patterns, with the main focus on recent developments. This review can be used both as an introduction to the fundamental modeling principles of human mobility, and as a collection of technical methods applicable to specific mobility-related problems. The review organizes the subject by differentiating between individual and population mobility and also between short-range and long-range mobility. Throughout the text the description of the theory is intertwined with real-world applications.},
  journal = {Physics Reports},
  doi = {10.1016/j.physrep.2018.01.001},
  author = {Barbosa, Hugo and Barthelemy, Marc and Ghoshal, Gourab and James, Charlotte R. and Lenormand, Maxime and Louail, Thomas and Menezes, Ronaldo and Ramasco, Jos{\'e} J. and Simini, Filippo and Tomasini, Marcello},
  month = mar,
  year = {2018},
  keywords = {Human dynamics,Human mobility,Origin–destination matrices,Random walks},
  pages = {1-74},
  file = {/Users/e1727/Dropbox/papers/storage/Barbosa et al_2018_Human mobility.pdf;/Users/e1727/Dropbox/papers/storage/Barbosa et al_2018_Human mobility2.pdf;/Users/e1727/Dropbox/Zotero/storage/R2KU2MJK/S037015731830022X.html}
}

@article{Henry1990Traffic,
  series = {{{IFAC}}/{{IFIP}}/{{IFORS Symposium}} on {{Control}}, {{Computers}}, {{Communications}} in {{Transportation}}, {{Paris}}, {{France}}, 19-21 {{September}}},
  title = {Traffic {{Congestion Control}}},
  volume = {23},
  issn = {1474-6670},
  abstract = {This survey paper presents the various urban traffic control strategies which have been proposed or applied to prevent and treat congestion. Some basic definitions about congestion, such as primary and secondary congestion, are remembered. Freeway control during congested situations is examined; the access control and exits control problems are developed. Approaches for intersection control are described: delay minimization, output flow rates maximization, LQ problem, congestion level feedback and democratic control. For network control the methods are classified into three classes. The first one concerns all systems which are based on application of rules rather than on a modelization of traffic; this class includes knowledge based systems. The second class of methods consider the static modelization of the traffic process and deals with flows. Methods for dynamic control of a network using queuing models are classified in the third class. Finally, some prospect is presented.},
  number = {2},
  journal = {IFAC Proceedings Volumes},
  doi = {10.1016/S1474-6670(17)52668-3},
  author = {Henry, J. J. and Farges, J. L.},
  month = sep,
  year = {1990},
  keywords = {optimal control,feedback,traffic control,Artificial intelligence,bang-bang control,centralized control,expert systems,flow control,hierarchical decision making,linear optimal control,linear programming,minimum principle,models,road traffic,saturation,saturation control,urban systems},
  pages = {177-182},
  file = {/Users/e1727/Dropbox/papers/storage/Henry_Farges_1990_Traffic Congestion Control.pdf;/Users/e1727/Dropbox/Zotero/storage/2DU679JF/S1474667017526683.html}
}

@book{wolsey2014integer,
  title = {Integer and Combinatorial Optimization},
  publisher = {{John Wiley \& Sons}},
  author = {Wolsey, Laurence A and Nemhauser, George L},
  year = {2014}
}


@article{Hamerlyeaau0823,
  title = {Experimental Investigation of Performance Differences between Coherent {{Ising}} Machines and a Quantum Annealer},
  volume = {5},
  abstract = {Physical annealing systems provide heuristic approaches to solving combinatorial optimization problems. Here, we benchmark two types of annealing machines\textemdash{}a quantum annealer built by D-Wave Systems and measurement-feedback coherent Ising machines (CIMs) based on optical parametric oscillators\textemdash{}on two problem classes, the Sherrington-Kirkpatrick (SK) model and MAX-CUT. The D-Wave quantum annealer outperforms the CIMs on MAX-CUT on cubic graphs. On denser problems, however, we observe an exponential penalty for the quantum annealer [exp(\textendash{$\alpha$}DWN2)] relative to CIMs [exp(\textendash{$\alpha$}CIMN)] for fixed anneal times, both on the SK model and on 50\% edge density MAX-CUT. This leads to a several orders of magnitude time-to-solution difference for instances with over 50 vertices. An optimal\textendash{}annealing time analysis is also consistent with a substantial projected performance difference. The difference in performance between the sparsely connected D-Wave machine and the fully-connected CIMs provides strong experimental support for efforts to increase the connectivity of quantum annealers.},
  number = {5},
  journal = {Science Advances},
  doi = {10.1126/sciadv.aau0823},
  author = {Hamerly, Ryan and Inagaki, Takahiro and McMahon, Peter L. and Venturelli, Davide and Marandi, Alireza and Onodera, Tatsuhiro and Ng, Edwin and Langrock, Carsten and Inaba, Kensuke and Honjo, Toshimori and Enbutsu, Koji and Umeki, Takeshi and Kasahara, Ryoichi and Utsunomiya, Shoko and Kako, Satoshi and Kawarabayashi, Ken-ichi and Byer, Robert L. and Fejer, Martin M. and Mabuchi, Hideo and Englund, Dirk and Rieffel, Eleanor and Takesue, Hiroki and Yamamoto, Yoshihisa},
  year = {2019},
  publisher = {{American Association for the Advancement of Science}},
  elocation-id = {eaau0823},
  eprint = {https://advances.sciencemag.org/content/5/5/eaau0823.full.pdf}
}

@article{Merle2019Turinglike,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1903.08506},
  primaryClass = {nlin, physics:physics},
  title = {Turing-like Patterns in an Asymmetric Dynamic {{Ising}} Model},
  abstract = {To investigate novel aspects of pattern formation in spin systems, we propose a mapping between reactive concentrations in a reaction-diffusion system and spin orientations in a dynamic multiple-spin Ising model. This specifically designed Ising model has asymmetric short-range interactions and several spin types coexisting at a site. The model is able to produce spatial patterns observed in reaction diffusion systems including Turing structures, showing that long-range interactions are not necessary to get such patterns in Ising models. While we used the example of genetic regulation during embryo-genesis to build our model, it can be used to study the behavior of other complex systems of interacting agents.},
  journal = {arXiv:1903.08506 [nlin, physics:physics]},
  author = {Merle, M{\'e}lody and Messio, Laura and Mozziconacci, Julien},
  month = mar,
  year = {2019},
  keywords = {Nonlinear Sciences - Adaptation and Self-Organizing Systems,Nonlinear Sciences - Pattern Formation and Solitons,Physics - Biological Physics},
  file = {/Users/e1727/Dropbox/papers/storage/Merle et al_2019_Turing-like patterns in an asymmetric dynamic Ising model.pdf;/Users/e1727/Dropbox/Zotero/storage/AULSAEZF/Merle et al. - 2019 - Turing-like patterns in an asymmetric dynamic Isin.pdf;/Users/e1727/Dropbox/Zotero/storage/D8PGP4WJ/1903.html}
}

@book{kuo1992digital,
  address = {{New York}},
  title = {Digital Control Systems},
  isbn = {0-19-512064-7},
  publisher = {{Oxford University Press}},
  author = {Kuo, Benjamin},
  year = {1992}
}

@article{Dumoulin2013Challenges,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1312.5258},
  primaryClass = {cs, stat},
  title = {On the {{Challenges}} of {{Physical Implementations}} of {{RBMs}}},
  abstract = {Restricted Boltzmann machines (RBMs) are powerful machine learning models, but learning and some kinds of inference in the model require sampling-based approximations, which, in classical digital computers, are implemented using expensive MCMC. Physical computation offers the opportunity to reduce the cost of sampling by building physical systems whose natural dynamics correspond to drawing samples from the desired RBM distribution. Such a system avoids the burn-in and mixing cost of a Markov chain. However, hardware implementations of this variety usually entail limitations such as low-precision and limited range of the parameters and restrictions on the size and topology of the RBM. We conduct software simulations to determine how harmful each of these restrictions is. Our simulations are designed to reproduce aspects of the D-Wave quantum computer, but the issues we investigate arise in most forms of physical computation.},
  journal = {arXiv:1312.5258 [cs, stat]},
  author = {Dumoulin, Vincent and Goodfellow, Ian J. and Courville, Aaron and Bengio, Yoshua},
  month = dec,
  year = {2013},
  keywords = {Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {/Users/e1727/Dropbox/papers/storage/Dumoulin et al_2013_On the Challenges of Physical Implementations of RBMs.pdf;/Users/e1727/Dropbox/Zotero/storage/5NAFIVA9/1312.html}
}

@inproceedings{Furtlehner2013AnIM,
  title = {An {{Ising Model}} for {{Road Traffic Inference}}},
  booktitle = {From {{Hamiltonian Chaos}} to {{Complex Systems}}: A {{Nonlinear Physics Approach}}},
  publisher = {{Springer}},
  author = {Furtlehner, Cyril},
  year = {2013},
  file = {/Users/e1727/Dropbox/papers/storage/An Ising Model for Road Traffic Inference Paper Microsoft Academic.pdf}
}

@article{Nagel1992cellular,
  title = {A Cellular Automaton Model for Freeway Traffic},
  volume = {2},
  copyright = {Les Editions de Physique},
  issn = {1155-4304, 1286-4862},
  abstract = {Journal de Physique I, Journal de Physique Archives repr{\'e}sente une mine d informations facile {\`a} consulter sur la mani{\`e}re dont la physique a {\'e}t{\'e} publi{\'e}e depuis 1872.},
  language = {en},
  number = {12},
  journal = {Journal de Physique I},
  doi = {10.1051/jp1:1992277},
  author = {Nagel, Kai and Schreckenberg, Michael},
  month = dec,
  year = {1992},
  pages = {2221-2229},
  file = {/Users/e1727/Dropbox/papers/storage/Nagel_Schreckenberg_1992_A cellular automaton model for freeway traffic.pdf;/Users/e1727/Dropbox/Zotero/storage/7Q3VD25B/jp1v2p2221.html}
}

@article{PhysRevE.51.2939,
  title = {Discrete Stochastic Models for Traffic Flow},
  volume = {51},
  number = {4},
  journal = {Phys. Rev. E},
  doi = {10.1103/PhysRevE.51.2939},
  author = {Schreckenberg, M. and Schadschneider, A. and Nagel, K. and Ito, N.},
  month = apr,
  year = {1995},
  pages = {2939-2949},
  file = {/Users/e1727/Dropbox/papers/storage/Discrete stochastic models for traffic flow.pdf},
  publisher = {{American Physical Society}},
  numpages = {0}
}

@book{mccoy2014two,
  title = {The Two-Dimensional {{Ising}} Model},
  publisher = {{Courier Corporation}},
  author = {McCoy, Barry M and Wu, Tai Tsun},
  year = {2014}
}

@article{binder1981finite,
  title = {Finite Size Scaling Analysis of {{Ising}} Model Block Distribution Functions},
  volume = {43},
  number = {2},
  journal = {Zeitschrift f{\"u}r Physik B Condensed Matter},
  author = {Binder, Kurt},
  year = {1981},
  pages = {119-140},
  publisher = {{Springer}}
}

@article{glauber1963time,
  title = {Time-Dependent Statistics of the {{Ising}} Model},
  volume = {4},
  number = {2},
  journal = {Journal of mathematical physics},
  author = {Glauber, Roy J},
  year = {1963},
  pages = {294-307},
  publisher = {{AIP}}
}

@article{yang1952spontaneous,
  title = {The Spontaneous Magnetization of a Two-Dimensional {{Ising}} Model},
  volume = {85},
  number = {5},
  journal = {Physical Review},
  author = {Yang, Chen Ning},
  year = {1952},
  pages = {808},
  publisher = {{APS}}
}

@article{doi:10.1002/cplx.20392,
  title = {Self-Organizing Traffic Lights at Multiple-Street Intersections},
  volume = {17},
  abstract = {Abstract The elementary cellular automaton following rule 184 can mimic particles flowing in one direction at a constant speed. Therefore, this automaton can model highway traffic qualitatively. In a recent paper, we have incorporated intersections regulated by traffic lights to this model using exclusively elementary cellular automata. In such a paper, however, we only explored a rectangular grid. We now extend our model to more complex scenarios using an hexagonal grid. This extension shows first that our model can readily incorporate multiple-way intersections and hence simulate complex scenarios. In addition, the current extension allows us to study and evaluate the behavior of two different kinds of traffic-light controller for a grid of six-way streets allowing for either two- or three-street intersections: a traffic light that tries to adapt to the amount of traffic (which results in self-organizing traffic lights) and a system of synchronized traffic lights with coordinated rigid periods (sometimes called the ``green-wave'' method). We observe a tradeoff between system capacity and topological complexity. The green-wave method is unable to cope with the complexity of a higher-capacity scenario, while the self-organizing method is scalable, adapting to the complexity of a scenario and exploiting its maximum capacity. Additionally, in this article, we propose a benchmark, independent of methods and models, to measure the performance of a traffic-light controller comparing it against a theoretical optimum. \textcopyright{} 2011 Wiley Periodicals, Inc. Complexity, 2012},
  number = {4},
  journal = {Complexity},
  doi = {10.1002/cplx.20392},
  author = {Gershenson, Carlos and Rosenblueth, David A.},
  year = {2012},
  keywords = {Self-organization,adaptation,elementary cellular automata,traffic lights},
  pages = {23-39},
  file = {/Users/e1727/Dropbox/papers/storage/Gershenson_Rosenblueth_2012_Self-organizing traffic lights at multiple-street intersections.pdf},
  eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cplx.20392}
}

@article{karypis1998fast,
  title = {A Fast and High Quality Multilevel Scheme for Partitioning Irregular Graphs},
  volume = {20},
  number = {1},
  journal = {SIAM Journal on scientific Computing},
  author = {Karypis, George and Kumar, Vipin},
  year = {1998},
  pages = {359-392},
  publisher = {{SIAM}}
}

@inproceedings{andersen2006local,
  title = {Local Graph Partitioning Using Pagerank Vectors},
  booktitle = {2006 47th {{Annual IEEE Symposium}} on {{Foundations}} of {{Computer Science}} ({{FOCS}}'06)},
  author = {Andersen, Reid and Chung, Fan and Lang, Kevin},
  year = {2006},
  pages = {475-486},
  organization = {{IEEE}}
}

@inproceedings{ding2001min,
  title = {A Min-Max Cut Algorithm for Graph Partitioning and Data Clustering},
  booktitle = {Proceedings 2001 {{IEEE International Conference}} on {{Data Mining}}},
  author = {Ding, Chris HQ and He, Xiaofeng and Zha, Hongyuan and Gu, Ming and Simon, Horst D},
  year = {2001},
  pages = {107-114},
  organization = {{IEEE}}
}

@inproceedings{stanton2012streaming,
  title = {Streaming Graph Partitioning for Large Distributed Graphs},
  booktitle = {Proceedings of the 18th {{ACM SIGKDD}} International Conference on {{Knowledge}} Discovery and Data Mining},
  author = {Stanton, Isabelle and Kliot, Gabriel},
  year = {2012},
  pages = {1222-1230},
  organization = {{ACM}}
}

@inproceedings{Tuna2006Shorter,
  title = {Shorter Horizons for Model Predictive Control},
  abstract = {We provide a less conservative (compared with our previous results) lower bound on the horizon length for a stabilizing model predictive control algorithm where the terminal cost is not assumed to be a local control Lyapunov function. Our main additional assumption is that the value function is bounded by a linear function of a measure of the state uniformly in the horizon length},
  booktitle = {2006 {{American Control Conference}}},
  doi = {10.1109/ACC.2006.1655466},
  author = {Tuna, S. E. and Messina, M. J. and Teel, A. R.},
  month = jun,
  year = {2006},
  keywords = {stability,Control systems,Constraint optimization,Cost function,Feedback loop,Length measurement,linear function,local control Lyapunov function,Lyapunov method,Lyapunov methods,model predictive control,Prediction algorithms,predictive control,Predictive control,Predictive models,Stability analysis,value function},
  pages = {6 pp.-},
  file = {/Users/e1727/Dropbox/papers/storage/Tuna et al_2006_Shorter horizons for model predictive control.pdf;/Users/e1727/Dropbox/Zotero/storage/4689E8WR/1655466.html}
}

@inproceedings{Ma2014onestep,
  title = {A One-Step Model Predictive Control for Modular Multilevel Converters},
  abstract = {Pulse Width Modulation (PWM) and Model Predictive Control (MPC) are two switching methods for Modular Mutlilevel Converter (MMC) presented in the literature [1], [2]. PWM switching cannot mitigate circulating currents in the converter bridges. An MPC method proposed in [2] compares all switching sequences and finds the optimal one to minimize the objective function (a weighted sum of the absolute values of the ac current deviation, capacitor voltage deviation, and the circulating current of the next time step). The computation effort is significant when the numbers of submodules increase. In this paper, a one-step model predictive control with minimum computing effort has been proposed to control the ac currents, keep the capacitor voltages nominal, and mitigate the circulating currents. The algorithm determines the ideal values of the lower-level and upper-level voltages on each phase based on the current state. The algorithm also determines which submodules to be switched on/off for the next time step according to the corresponding upper/lower current. The performance of the proposed method is evaluated via simulation in Matlab SimPowerSystems. The PWM and the proposed MPC are compared for their control effort and performance.},
  booktitle = {2014 {{IEEE PES General Meeting}} | {{Conference Exposition}}},
  doi = {10.1109/PESGM.2014.6939209},
  author = {Ma, Y. and Miao, Z. and Disfani, V. R. and Fan, L.},
  month = jul,
  year = {2014},
  keywords = {Switches,Mathematical model,predictive control,Predictive control,AC current control,AC current deviation,capacitor voltage deviation,Capacitors,circulating current mitigation,converter bridges,Converters,electric current control,lower-level voltages,Matlab SimPowerSystems,MMC,Model Predictive Control,Modular Multilevel Converter,modular multilevel converters,MPC method,nominal capacitor voltage,objective function minimization,one-step model predictive control,pulse width modulation,Pulse width modulation,Pulse Width Modulation,PWM power convertors,PWM switching,switching method,switching sequences,upper-level voltages,Voltage control},
  pages = {1-5},
  file = {/Users/e1727/Dropbox/papers/storage/Ma et al_2014_A one-step model predictive control for modular multilevel converters.pdf;/Users/e1727/Dropbox/Zotero/storage/HNVZDKKG/6939209.html}
}

@article{Wei2019Survey,
  archivePrefix = {arXiv},
  eprinttype = {arxiv},
  eprint = {1904.08117},
  primaryClass = {cs, stat},
  title = {A {{Survey}} on {{Traffic Signal Control Methods}}},
  abstract = {Traffic signal control is an important and challenging real-world problem, which aims to minimize the travel time of vehicles by coordinating their movements at the road intersections. Current traffic signal control systems in use still rely heavily on oversimplified information and rule-based methods, although we now have richer data, more computing power and advanced methods to drive the development of intelligent transportation. With the growing interest in intelligent transportation using machine learning methods like reinforcement learning, this survey covers the widely acknowledged transportation approaches and a comprehensive list of recent literature on reinforcement for traffic signal control. We hope this survey can foster interdisciplinary research on this important topic.},
  journal = {arXiv:1904.08117 [cs, stat]},
  author = {Wei, Hua and Zheng, Guanjie and Gayah, Vikash and Li, Zhenhui},
  month = apr,
  year = {2019},
  keywords = {68Txx,Computer Science - Artificial Intelligence,Computer Science - Machine Learning,Statistics - Machine Learning},
  file = {/Users/e1727/Dropbox/papers/storage/Wei et al_2019_A Survey on Traffic Signal Control Methods.pdf;/Users/e1727/Dropbox/Zotero/storage/Q6M6EU2R/1904.html}
}

@article{Papageorgiou2003Review,
  title = {Review of Road Traffic Control Strategies},
  volume = {91},
  issn = {0018-9219},
  abstract = {Traffic congestion in urban road and freeway networks leads to a strong degradation of the network infrastructure and accordingly reduced throughput, which can be countered via suitable control measures and strategies. After illustrating the main reasons for infrastructure deterioration due to traffic congestion, a comprehensive overview of proposed and implemented control strategies is provided for three areas: urban road networks, freeway networks, and route guidance. Selected application results, obtained from either simulation studies or field implementations, are briefly outlined to illustrate the impact of various control actions and strategies. The paper concludes with a brief discussion of future needs in this important technical area.},
  number = {12},
  journal = {Proceedings of the IEEE},
  doi = {10.1109/JPROC.2003.819610},
  author = {Papageorgiou, M. and Diakaki, C. and Dinopoulou, V. and Kotsialos, A. and {Yibing Wang}},
  month = dec,
  year = {2003},
  keywords = {automated highways,Communication system traffic control,Control systems,Degradation,Delay,driver information,Economic forecasting,freeway network control,intelligent transportation systems,Intelligent transportation systems,ramp metering,reviews,road traffic,Roads,route guidance,Throughput,Traffic control,traffic signal control,transportation,urban network control,Vehicles},
  pages = {2043-2067},
  file = {/Users/e1727/Dropbox/papers/storage/Papageorgiou et al_2003_Review of road traffic control strategies.pdf;/Users/e1727/Dropbox/Zotero/storage/ZMLCTD3D/Papageorgiou et al. - 2003 - Review of road traffic control strategies.pdf;/Users/e1727/Dropbox/Zotero/storage/P9RE6EZC/1246386.html}
}

@techreport{koonce2008traffic,
  title = {Traffic Signal Timing Manual.},
  institution = {{United States. Federal Highway Administration}},
  author = {Koonce, Peter and Rodegerdts, Lee},
  year = {2008}
}

@book{roess2004traffic,
  title = {Traffic Engineering},
  publisher = {{Pearson/Prentice Hall}},
  author = {Roess, Roger P and Prassas, Elena S and McShane, William R},
  year = {2004}
}

@incollection{varaiya2013max,
  title = {The Max-Pressure Controller for Arbitrary Networks of Signalized Intersections},
  booktitle = {Advances in {{Dynamic Network Modeling}} in {{Complex Transportation Systems}}},
  publisher = {{Springer}},
  author = {Varaiya, Pravin},
  year = {2013},
  pages = {27-66}
}

@article{lowrie1990scats,
  title = {{{SCATS}}-{{A}} Traffic Responsive Method of Controlling Urban Traffic},
  journal = {Sales information brochure published by Roads \& Traffic Authority, Sydney, Australia},
  author = {Lowrie, P},
  year = {1990}
}

@article{arel2010reinforcement,
  title = {Reinforcement Learning-Based Multi-Agent System for Network Traffic Signal Control},
  volume = {4},
  number = {2},
  journal = {IET Intelligent Transport Systems},
  author = {Arel, Itamar and Liu, Cong and Urbanik, T and Kohls, AG},
  year = {2010},
  pages = {128-135},
  file = {/Users/e1727/Dropbox/papers/storage/Arel et al_2010_Reinforcement learning-based multi-agent system for network traffic signal.pdf},
  publisher = {{IET}}
}

@article{mousavi2017traffic,
  title = {Traffic Light Control Using Deep Policy-Gradient and Value-Function-Based Reinforcement Learning},
  volume = {11},
  number = {7},
  journal = {IET Intelligent Transport Systems},
  author = {Mousavi, Seyed Sajad and Schukat, Michael and Howley, Enda},
  year = {2017},
  pages = {417-423},
  file = {/Users/e1727/Dropbox/papers/storage/Mousavi et al_2017_Traffic light control using deep policy-gradient and value-function-based.pdf},
  publisher = {{IET}}
}

@inproceedings{khamis2012multi,
  title = {Multi-Objective Traffic Light Control System Based on {{Bayesian}} Probability Interpretation},
  booktitle = {2012 15th {{International IEEE Conference}} on {{Intelligent Transportation Systems}}},
  author = {Khamis, Mohamed A and Gomaa, Walid and {El-Shishiny}, Hisham},
  year = {2012},
  pages = {995-1000},
  file = {/Users/e1727/Dropbox/papers/storage/Khamis et al_2012_Multi-objective traffic light control system based on Bayesian probability.pdf},
  organization = {{IEEE}}
}

@inproceedings{nishi2018traffic,
  title = {Traffic {{Signal Control Based}} on {{Reinforcement Learning}} with {{Graph Convolutional Neural Nets}}},
  booktitle = {2018 21st {{International Conference}} on {{Intelligent Transportation Systems}} ({{ITSC}})},
  author = {Nishi, Tomoki and Otaki, Keisuke and Hayakawa, Keiichiro and Yoshimura, Takayoshi},
  year = {2018},
  pages = {877-883},
  organization = {{IEEE}}
}



